A complete tree-level dictionary between simplified BSM models and SMEFT (d $\leq$ 7) operators

Finding all possible UV resonances of effective operators is an important task in the bottom-up approach of effective field theory. We present all the tree-level UV resonances for the dimension-5, -6 and -7 operators in the Standard Model effective field theory (SMEFT), and then obtain the correspondence between the UV resonances and the effective operators from the relations among their Wilson coefficients, through the functional matching and operator reduction procedure. This provides a cross-dimension UV/IR dictionary for the SMEFT at tree-level, and the methods used here, especially the on-shell construction of general UV Lagrangian and the systematic reduction of operators, are extendable for UV resonances of $d \geq 8$ operators in SMEFT and other EFTs.

==> chapters/app_notation.tex <==
\section{Transformation of gauge notation}
\label{sec:gaugenot}

\paragraph{$SU(3)$ group}
\begin{itemize}
    \item $\mathbf{3}, \mathbf{\overline{3}}$ representations
    \item $\mathbf{8}$ representations
        \begin{equation}
            \phi_a^b = \frac{1}{\sqrt{2}}\phi^A (\lambda^A)_a^b
        \end{equation}
    \item $\mathbf{6}, \mathbf{\overline{6}}$ representations
        \begin{equation}
            \phi_{ab} = (D^{\frak{a}})_{ab} \phi_{\frak{a}}, \phi^{\dagger ab} = (D_{\frak{a}})^{ab} \phi^{\dagger\frak{a}}
        \end{equation}
\end{itemize}
where $(D^{\frak{a}})_{ab} = (D_{\frak{a}})^{ab}$ and
\begin{align}
	(D_1)^{ab} = \left( \begin{array}{ccc}
		1 & 0 & 0 \\
		0 & 0 & 0 \\
		0 & 0 & 0
	\end{array}\right),
	%
	(D_2)^{ab} = \left( \begin{array}{ccc}
		0 & 0 & 0 \\
		0 & 1 & 0 \\
		0 & 0 & 0
	\end{array}\right),
	%
	(D_3)^{ab} = \left( \begin{array}{ccc}
		0 & 0 & 0 \\
		0 & 0 & 0 \\
		0 & 0 & 1
	\end{array}\right), \nonumber\\
	%
	(D_4)^{ab} = \frac{1}{\sqrt 2}\left( \begin{array}{ccc}
		0 & 0 & 0 \\
		0 & 0 & 1 \\
		0 & 1 & 0
	\end{array}\right),
	%
	(D_5)^{ab} = \frac{1}{\sqrt 2}\left( \begin{array}{ccc}
		0 & 0 & 1 \\
		0 & 0 & 0 \\
		1 & 0 & 0
	\end{array}\right),
	%
	(D_6)^{ab} = \frac{1}{\sqrt 2}\left( \begin{array}{ccc}
		0 & 1 & 0 \\
		1 & 0 & 0 \\
		0 & 0 & 0
	\end{array}\right).
\end{align}


\paragraph{$SU(2)$ group}
\begin{itemize}
    \item $\mathbf{2}, \mathbf{\overline{2}}$ representations
    \item $\mathbf{3}$ representations
        \begin{equation}
            \phi_{ij} = \frac{1}{\sqrt{2}}\phi^I (\tau^I\epsilon)_{ij}, \phi^{\dagger ij} = (\phi_{ij})^\dagger = \frac{1}{\sqrt{2}}\phi^I (\tau^I)_k^i \epsilon^{kj}.
        \end{equation}
    \item $\mathbf{4}, \mathbf{\overline{4}}$ representations
\end{itemize}

Rising and descending of the indices for real fields:
\begin{equation}
    \phi^{i_1\cdots i_{2n}} = (-1)^{n}\epsilon^{i_1j_1}\cdots\epsilon^{i_{2n}j_{2n}}\phi_{j_1\cdots j_{2n}},\\
    \phi_{i_1\cdots i_{2n}} = (-1)^{n}\epsilon_{i_1j_1}\cdots\epsilon_{i_{2n}j_{2n}}\phi^{j_1\cdots j_{2n}}
\end{equation}


%%%%%%%%%%%%%%%%%%%%


% \section{The UV Lagrangian in two-component notation}
% \label{sec:lagintwo}





==> result/eftdim6.tex <==
\begin{align}
\begin{autobreak}
 {Q_{5}} =
 
-\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{2 {M_{F_{1}}}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi }} =
 \frac{2 \lambda_H (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}}}{{M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}}}{3 {M_{S_{7}}^2}}
+\frac{4 \lambda_H \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{8 \lambda_H \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{1}S_{1}}}^{{p_1p_2}}}{{M_{S_{1}}^4}}
-\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{HH^\dagger S_{1}S_{5}}}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(1)}}^{{p_2p_1}}}{4 {M_{S_{5}}^4}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(2)}}^{{p_2p_1}}}{2 {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_2p_1}}}{{M_{S_{6}}^4}}
+\frac{8 \lambda_H \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}}}{{M_{S_{1}}^4} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1*}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1*}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_3}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3*}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1*}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_1}}}{4 {M_{S_{4}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{1}S_{1}}}^{{p_1p_2p_3}}}{{M_{S_{1}}^6}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{5}S_{5}}}^{{p_1p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi box}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}})^2}{2 {M_{S_{1}}^4}}
+\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{4 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi D}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
+\frac{4 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
-\frac{4 \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{e\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{p_1p_2}}}{2 {M_{F_{3}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{p_1p_2}}}{2 {M_{F_{4}}^2}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2p_1}}}{2 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{3L}H}}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{3}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{4L}H^\dagger }}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{4}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}}}{{M_{F_{3}}} {M_{F_{5}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{2 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}F_{6R}^\dagger H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{4}}} {M_{F_{6}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1}}}{4 {M_{F_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{2R}^\dagger S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{2}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{6R}^\dagger S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{6}}} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{u\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2p_1}}}{{M_{F_{11}}^2}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2p_1}}}{{M_{F_{12}}^2}}
-\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{14L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{14}}}}
+\frac{{y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{9L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{9}}}}
-\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{9L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{9}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{9}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{F_{9L}S_{1}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{9}}} {M_{S_{1}}^2}}
+\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
+\frac{2 \mathcal{D}_{{F_{14L}S_{5}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{14}}} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
-\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{d\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{p_1p_2}}}{{M_{F_{10}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{p_1p_2}}}{{M_{F_{11}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{13L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{13}}}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{{y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{8L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{8}}}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{8L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{8}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(2)}}^{{p_1*}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{8L}S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{8}}} {M_{S_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{13L}S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{13}}} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}}
+\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi l1}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
-\frac{3 \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi l3}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{2 {M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi e}} =
 \frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}}}{2 {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}}}{2 {M_{F_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi q1}} =
 
-\frac{3 \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{3 \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
+\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi q3}} =
 \frac{\mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{\mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
-\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi u}} =
 
-\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_4*}}}{{M_{F_{11}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_4*}}}{{M_{F_{12}}^2}}
+\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi d}} =
 \frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}}}{{M_{F_{10}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}}}{{M_{F_{11}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{\phi ud}} =
 \frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}}}{{M_{F_{11}}^2}}
+\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_1p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ll}} =
 
-\frac{\mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_4p_1}}}{4 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_3p_1}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qq1}} =
 \frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
-\frac{2 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{3 \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
+\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qq3}} =
 
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_4p_1}}}{3 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{lq1}} =
 \frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{3 \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{lq3}} =
 
-\frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
+\frac{\mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ee}} =
 \frac{\mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_4f_3p_1*}}}{2 {M_{S_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{uu}} =
 
-\frac{2 \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
-\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{dd}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{eu}} =
 
-\frac{4 \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_1f_4p_1*}} \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_3f_2p_1}}}{{M_{V_{6}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ed}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_3f_2p_1*}}}{{M_{V_{5}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_3f_4p_1*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ud1}} =
 
-\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{16}}^2}}
-\frac{128 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{9 {M_{V_{13}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ud8}} =
 
-\frac{32 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{13}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{le}} =
 \frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{lu}} =
 \frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{4 \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ld}} =
 \frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_3f_4p_1*}}}{{M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qe}} =
 \frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qu1}} =
 \frac{4 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{32 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{11}}^2}}
+\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{3 {M_{V_{7}}^2}}
-\frac{16 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qu8}} =
 \frac{16 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{11}}^2}}
-\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}}
+\frac{4 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qd1}} =
 \frac{32 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{3 {M_{V_{10}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{3 {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{64 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qd8}} =
 \frac{16 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{10}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{ledq}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_3p_1}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{quqd1}} =
 \frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{3 {M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{quqd8}} =
 \frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{19}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{{M_{S_{10}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{{M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{lequ1}} =
 
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{13}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{lequ3}} =
 \frac{\mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{2 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{2 {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{duq}} =
 
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_1p_1*}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qqu}} =
 \frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_1p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{qqq}} =
 \frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_3p_1}}}{{M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_3f_2p_1}}}{{M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{duu}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_3f_4*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_3*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {Q_{LH}} =
 
-\frac{{C}_5^{{f_1f_2}} (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
-\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
-\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
-\frac{2 {C}_5^{{f_1f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
+\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
-\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}}}{2 {M_{F_{1}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}}}{2 {M_{F_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}}}{2 {M_{V_{4}}^2}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}}}{4 {M_{F_{5}}^2}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}}}{2 {M_{F_{6}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}}}{4 {M_{F_{5}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}}}{2 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}


==> result/eftdim7_dag.tex <==
\subsection{Dimension-5}
\begin{align}
\begin{autobreak}
 {O_{5}} =
 
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mu_H^2 }{2 {M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mu_H^2 }{4 {M_{F_{5}}^3}}
-\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{2 {M_{F_{1}}}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{5}^\dagger } =
 
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mu_H^2 }{2 {M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mu_H^2 }{4 {M_{F_{5}}^3}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{2 {M_{F_{1}}}}
-\frac{\mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{4 {M_{F_{5}}}} 
\end{autobreak}
\end{align}

\subsection{Dimension-6}
\begin{align}
\begin{autobreak}
 {O_{\phi }} =
 \frac{2 \lambda_H (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}}}{{M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}}}{3 {M_{S_{7}}^2}}
+\frac{4 \lambda_H \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{4 \lambda_H \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}}}{{M_{V_{15}}^2}}
-\frac{8 \lambda_H \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{1}S_{1}}}^{{p_1p_2}}}{{M_{S_{1}}^4}}
-\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{HH^\dagger S_{1}S_{5}}}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(1)}}^{{p_2p_1}}}{4 {M_{S_{5}}^4}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(2)}}^{{p_2p_1}}}{2 {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_2p_1}}}{{M_{S_{6}}^4}}
+\frac{8 \lambda_H \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}}}{{M_{S_{1}}^4} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1*}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1*}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_3}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3*}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1*}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_1}}}{4 {M_{S_{4}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{1}S_{1}}}^{{p_1p_2p_3}}}{{M_{S_{1}}^6}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{5}S_{5}}}^{{p_1p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi box}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}})^2}{2 {M_{S_{1}}^4}}
+\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{4 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi D}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}}}{{M_{V_{15}}^2}}
+\frac{4 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
-\frac{4 \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{e\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{p_1p_2}}}{2 {M_{F_{3}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{p_1p_2}}}{2 {M_{F_{4}}^2}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2p_1}}}{2 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{3L}H}}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{3}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{4L}H^\dagger }}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{4}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}}}{{M_{F_{3}}} {M_{F_{5}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{2 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}F_{6R}^\dagger H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{4}}} {M_{F_{6}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1}}}{4 {M_{F_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{2R}^\dagger S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{2}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{6R}^\dagger S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{6}}} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{e\phi }^\dagger } =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{e}}^{{f_1f_2*}}}{2 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_1f_2*}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{e}}^{{f_1f_2*}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_1f_2*}}}{2 {M_{V_{4}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{e}}^{{f_1f_2*}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{e}}^{{f_1f_2*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_1f_2*}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_1f_2*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{e}}^{{f_1f_2*}}}{{M_{V_{4}}^2}}
+\frac{{y}_{{e}}^{{p_1f_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_2}}}{2 {M_{F_{3}}^2}}
+\frac{{y}_{{e}}^{{p_1f_2*}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_2}}}{2 {M_{F_{4}}^2}}
+\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_2}}}{2 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_2}} \mathcal{D}_{{F_{2R}^\dagger F_{3L}H}}^{{p_2p_1}}}{{M_{F_{2}}} {M_{F_{3}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_2}} \mathcal{D}_{{F_{2R}^\dagger F_{4L}H^\dagger }}^{{p_2p_1}}}{{M_{F_{2}}} {M_{F_{4}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{{M_{F_{3}}} {M_{F_{5}}}}
+\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{2 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{2 {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}F_{6R}^\dagger H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{2 {M_{F_{4}}} {M_{F_{6}}}}
+\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{4 {M_{F_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{2R}^\dagger S_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{2}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{6R}^\dagger S_{5}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{6}}} {M_{S_{5}}^2}}
-\frac{i {y}_{{e}}^{{p_1f_2*}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{e}}^{{p_1f_2*}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{i {y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2p_1p_2}}}{2 {M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{u\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2p_1}}}{{M_{F_{11}}^2}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2p_1}}}{{M_{F_{12}}^2}}
-\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{14L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{14}}}}
+\frac{{y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{9L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{9}}}}
-\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{9L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{9}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{9}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{F_{9L}S_{1}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{9}}} {M_{S_{1}}^2}}
+\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
+\frac{2 \mathcal{D}_{{F_{14L}S_{5}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{14}}} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
-\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{u\phi }^\dagger } =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{u}}^{{f_2f_1*}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_2f_1*}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{u}}^{{f_2f_1*}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_2f_1*}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{u}}^{{f_2f_1*}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{u}}^{{f_2f_1*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_2f_1*}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_2f_1*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{u}}^{{f_2f_1*}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{u}}^{{p_1f_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_2}}}{{M_{F_{11}}^2}}
+\frac{2 {y}_{{u}}^{{p_1f_1*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_2}}}{{M_{F_{12}}^2}}
-\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{2 {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{13}}^2}}
+\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger F_{14L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{12}}} {M_{F_{14}}}}
+\frac{{y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{11R}^\dagger F_{9L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{11}}} {M_{F_{9}}}}
-\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger F_{9L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{12}}} {M_{F_{9}}}}
+\frac{2 {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2p_1*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_1}}}{{M_{F_{9}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{F_{9L}S_{1}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{9}}} {M_{S_{1}}^2}}
-\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
-\frac{2 \mathcal{D}_{{F_{14L}S_{5}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{14}}} {M_{S_{5}}^2}}
-\frac{2 i {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
-\frac{2 i {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1p_1p_2}}}{{M_{V_{4}}^2}}
+\frac{i {y}_{{u}}^{{f_2p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1p_1p_2}}}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{2 i {y}_{{u}}^{{p_1f_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}}
-\frac{2 i {y}_{{u}}^{{p_1f_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{d\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{p_1p_2}}}{{M_{F_{10}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{p_1p_2}}}{{M_{F_{11}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{13L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{13}}}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{{y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{8L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{8}}}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{8L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{8}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{8L}S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{8}}} {M_{S_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{13L}S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{13}}} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}}
+\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{d\phi }^\dagger } =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{d}}^{{f_1f_2*}}}{2 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_1f_2*}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{d}}^{{f_1f_2*}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_1f_2*}}}{2 {M_{V_{4}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{d}}^{{f_1f_2*}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{d}}^{{f_1f_2*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_1f_2*}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_1f_2*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{d}}^{{f_1f_2*}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{d}}^{{p_1f_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{p_1p_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_2}}}{{M_{F_{10}}^2}}
+\frac{2 {y}_{{d}}^{{p_1f_2*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_2}}}{{M_{F_{11}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger F_{13L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{10}}} {M_{F_{13}}}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{{y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{13}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_2}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{2 {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_2}}}{{M_{F_{14}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger F_{8L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{10}}} {M_{F_{8}}}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11R}^\dagger F_{8L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{11}}} {M_{F_{8}}}}
+\frac{2 {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{8L}S_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{8}}} {M_{S_{1}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{13L}S_{5}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{13}}} {M_{S_{5}}^2}}
-\frac{2 i {y}_{{d}}^{{p_1f_2*}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
-\frac{2 i {y}_{{d}}^{{p_1f_2*}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1p_1p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{2 i {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}}
-\frac{2 i {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2p_1p_2}}}{{M_{V_{4}}^2}}
-\frac{i {y}_{{d}}^{{f_1p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2p_1p_2}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi l1}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
-\frac{3 \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi l3}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{2 {M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi e}} =
 \frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}}}{2 {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}}}{2 {M_{F_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi q1}} =
 
-\frac{3 \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{3 \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
+\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi q3}} =
 \frac{\mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{\mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
-\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi u}} =
 
-\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_4*}}}{{M_{F_{11}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_4*}}}{{M_{F_{12}}^2}}
+\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi d}} =
 \frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}}}{{M_{F_{10}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}}}{{M_{F_{11}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi ud}} =
 \frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}}}{{M_{F_{11}}^2}}
+\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_1p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi ud}^\dagger } =
 \frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_4*}}}{{M_{F_{11}}^2}}
-\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ll}} =
 
-\frac{\mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_4p_1}}}{4 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_3p_1}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qq1}} =
 \frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
-\frac{2 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{3 \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
+\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qq3}} =
 
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_4p_1}}}{3 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lq1}} =
 \frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{3 \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lq3}} =
 
-\frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
+\frac{\mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ee}} =
 \frac{\mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_4f_3p_1*}}}{2 {M_{S_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{uu}} =
 
-\frac{2 \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
-\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dd}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eu}} =
 
-\frac{4 \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_1f_4p_1*}} \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_3f_2p_1}}}{{M_{V_{6}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ed}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_3f_2p_1*}}}{{M_{V_{5}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_3f_4p_1*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ud1}} =
 
-\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{16}}^2}}
-\frac{128 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{9 {M_{V_{13}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ud8}} =
 
-\frac{32 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{13}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{le}} =
 \frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lu}} =
 \frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{4 \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ld}} =
 \frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_3f_4p_1*}}}{{M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qe}} =
 \frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qu1}} =
 \frac{4 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{32 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{11}}^2}}
+\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{3 {M_{V_{7}}^2}}
-\frac{16 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qu8}} =
 \frac{16 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{11}}^2}}
-\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}}
+\frac{4 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qd1}} =
 \frac{32 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{3 {M_{V_{10}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{3 {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{64 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qd8}} =
 \frac{16 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{10}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ledq}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_3p_1}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ledq}^\dagger } =
 
-\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_3f_1p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_2f_4p_1*}}}{{M_{V_{5}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_2p_1*}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_1f_4p_1*}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd1}} =
 \frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{3 {M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd1}^\dagger } =
 \frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4}}}{{M_{S_{4}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1}}}{3 {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1}}}{3 {M_{S_{10}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1}}}{3 {M_{S_{16}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1}}}{3 {M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd8}} =
 \frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{19}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{{M_{S_{10}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{{M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd8}^\dagger } =
 \frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4}}}{{M_{S_{19}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1}}}{{M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1}}}{{M_{S_{16}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1}}}{{M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ1}} =
 
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{13}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ1}^\dagger } =
 
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4}}}{{M_{S_{13}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ3}} =
 \frac{\mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{2 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{2 {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ3}^\dagger } =
 \frac{\mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1}}}{2 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4}}}{2 {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duq}} =
 
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_1p_1*}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duq}^\dagger } =
 
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_3p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_4f_2p_1*}}}{{M_{V_{7}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqu}} =
 \frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_1p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqu}^\dagger } =
 \frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqq}} =
 \frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_3p_1}}}{{M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_3f_2p_1}}}{{M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqq}^\dagger } =
 \frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QQS_{14}}}^{{f_3f_4p_1*}}}{{M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{{M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duu}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_3f_4*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_3*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duu}^\dagger } =
 \frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_3f_4}}}{{M_{S_{9}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3}}}{{M_{S_{9}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_2p_1f_3}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}

\subsection{Dimension-7}
\begin{align}
\begin{autobreak}
 {O_{LH}} =
 
-\frac{{C}_5^{{f_1f_2}} (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
-\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
-\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{\lambda_H \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}^3}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{2 {M_{F_{1}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{2 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_3p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_3f_1}}}{{M_{F_{1}}^2} {M_{F_{3}}}}
+\frac{\lambda_H \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{2 {M_{F_{5}}^3}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{5}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{5}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_3p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{3 {M_{F_{5}}^2} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}}}{{M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{2 {M_{F_{6}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{2 {M_{F_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
-\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
+\frac{5 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_1}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_2}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2}}}{2 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_1p_2}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_2}}}{{M_{F_{6}}} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{2 {C}_5^{{f_1f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_2p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{3 {M_{F_{6}}} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_2p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{2 {C}_5^{{f_1f_2}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}}}{{M_{V_{15}}^2}}
+\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{1}S_{1}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{{M_{F_{1}}^2} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{5}S_{1}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{5}}^2} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{7L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{3 {M_{F_{7}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{5}S_{5}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_3p_2}}}{{M_{F_{6}}} {M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_2p_1p_3}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_2p_1p_3}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LH}^\dagger } =
 
-\frac{{C}_5^{{f_5f_6*}} (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
-\frac{2 {C}_5^{{f_5f_6*}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{2 {C}_5^{{f_5f_6*}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
-\frac{{C}_5^{{f_5f_6*}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
+\frac{{C}_5^{{f_5f_6*}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{\lambda_H \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}}}{{M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_3p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_3f_6*}}}{{M_{F_{1}}^2} {M_{F_{3}}}}
-\frac{{C}_5^{{f_6p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^2}}
-\frac{{C}_5^{{p_1f_6*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^2}}
+\frac{\lambda_H \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}}}{2 {M_{F_{5}}^3}}
+\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_5*}}}{{M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_5*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_3p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}}}{3 {M_{F_{5}}^2} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}}}{4 {M_{F_{3}}} {M_{F_{5}}^2}}
-\frac{{C}_5^{{f_6p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^2}}
-\frac{{C}_5^{{p_1f_6*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^2}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_6*}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
+\frac{5 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_5*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
-\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_6*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
-\frac{{C}_5^{{f_6p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1}}}{2 {M_{F_{6}}^2}}
-\frac{{C}_5^{{p_1f_6*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1}}}{2 {M_{F_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_5*}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2*}}}{2 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_6*}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_6p_2*}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_2*}}}{{M_{F_{6}}} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_5p_2*}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2*}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_6p_2*}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2*}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_5p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_6p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_5p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_6*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_6p_3*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_6*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_5p_3*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_6*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_6*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_5p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}}}{3 {M_{F_{6}}} {M_{F_{7}}} {M_{S_{6}}^2}}
-\frac{2 {C}_5^{{f_5f_6*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
+\frac{2 {C}_5^{{f_5f_6*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}}}{{M_{V_{15}}^2}}
+\frac{4 {C}_5^{{f_5f_6*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_6p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_5p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_5p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{1}S_{1}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{{M_{F_{1}}^2} {M_{S_{1}}^2}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_5p_3*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{5}S_{1}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{5}}^2} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_6p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_6*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{7L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_6p_3*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{3 {M_{F_{7}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_5p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{5}S_{5}}}^{{p_1p_2p_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_5p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_6p_3*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{4 {C}_5^{{f_5f_6*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2*}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2*}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2*}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2*}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_3p_2*}}}{{M_{F_{6}}} {M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_6*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_6p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_2*}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_3p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{i {C}_5^{{f_6p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{p_1f_6*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{f_6p_1*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{p_1f_6*}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {C}_5^{{f_6p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {C}_5^{{p_1f_6*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{f_6p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{p_1f_6*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_2p_3p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_6f_5p_3*}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_2p_3p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LeHD}} =
 
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^3}}
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{LLS_{6}}}^{{f_1p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{S_{6}}^4}}
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^3}}
+\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_1p_2}}}{{M_{S_{6}}^4}}
+\frac{2 i \mathcal{D}_{{eF_{1}V_{2}}}^{{f_5p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{{M_{F_{1}}} {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{{M_{F_{3}}} {M_{F_{5}}^2}}
+\frac{2 i \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{2 {M_{F_{3}}^2} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{3}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_5p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{5}}^2} {M_{S_{6}}^2}}
-\frac{2 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_5f_1p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{HS_{6}V_{3}^\dagger D}}^{{p_2p_1}}}{{M_{S_{6}}^2} {M_{V_{3}}^2}}
-\frac{4 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_5f_1p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_2p_1}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LeHD}^\dagger } =
 
-\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}}}{2 {M_{F_{5}}^3}}
-\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_5p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{S_{6}}^4}}
+\frac{{y}_{{e}}^{{f_1p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_5p_2*}}}{{M_{S_{6}}^4}}
-\frac{2 i \mathcal{D}_{{eF_{1}V_{2}}}^{{f_1p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2*}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}}}{{M_{F_{1}}} {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}}}{{M_{F_{3}}} {M_{F_{5}}^2}}
-\frac{2 i \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_1f_5p_2}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2*}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}}}{2 {M_{F_{3}}^2} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{3}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{5}}^2} {M_{S_{6}}^2}}
+\frac{2 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_5p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{D}_{{HS_{6}V_{3}^\dagger D}}^{{p_2p_1*}}}{{M_{S_{6}}^2} {M_{V_{3}}^2}}
+\frac{4 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2*}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_2p_1*}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD1}} =
 \frac{2 \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{{M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD1}^\dagger } =
 \frac{2 \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{{M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD2}} =
 
-\frac{4 \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{2 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD2}^\dagger } =
 
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{{M_{F_{1}}^3}}
-\frac{4 \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{2 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHB}} =
 
-\frac{i {g'} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{8 {M_{F_{1}}^3}}
-\frac{i {g'} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{2 {M_{S_{6}}^4}}
-\frac{i {g'} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{16 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHB}^\dagger } =
 \frac{i {g'} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{8 {M_{F_{1}}^3}}
+\frac{i {g'} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{2 {M_{S_{6}}^4}}
+\frac{i {g'} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{16 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHW}} =
 
-\frac{i {g} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{8 {M_{F_{1}}^3}}
-\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{4 {M_{S_{6}}^4}}
+\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{4 {M_{S_{6}}^4}}
+\frac{3 i {g} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{16 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHW}^\dagger } =
 \frac{i {g} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{8 {M_{F_{1}}^3}}
-\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{4 {M_{S_{6}}^4}}
+\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{4 {M_{S_{6}}^4}}
{\xuxiang{+\frac{13 i {g} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{16 {M_{F_{5}}^3}} }}
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eLLLH}} =
 
-\frac{{y}_{{e}}^{{f_1f_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4}}}{2 {M_{F_{1}}^3}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{3 \mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{{y}_{{e}}^{{f_1f_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4}}}{4 {M_{F_{5}}^3}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_3p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_4}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_3p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_4p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{F_{4}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{F_{4}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{2 {M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{2 {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{2 {M_{F_{4}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{2 {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_2p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{5 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eLLLH}^\dagger } =
 
-\frac{{y}_{{e}}^{{f_5f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{2 {M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_4p_1*}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{{y}_{{e}}^{{f_5f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{4 {M_{F_{5}}^3}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1*}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_4p_1*}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_5p_1*}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_5p_1*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2*}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2*}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{3 \mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_2*}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_2p_1*}} \mathcal{D}_{{F_{4L}LS_{2}^\dagger }}^{{p_1f_3p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_2*}}}{{M_{F_{4}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_2*}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_2p_1*}} \mathcal{D}_{{F_{4L}LS_{2}^\dagger }}^{{p_1f_3p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_2*}}}{{M_{F_{4}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_2p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{5 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_2p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_3p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}}}{2 {M_{F_{4}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_2p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_3p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}}}{2 {M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_2f_3p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH1}} =
 
-\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{{M_{F_{1}}^3}}
-\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{2 {M_{F_{5}}^3}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{1}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH1}^\dagger } =
 
-\frac{{y}_{{d}}^{{f_5f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{{M_{F_{1}}^3}}
-\frac{{y}_{{d}}^{{f_5f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{2 {M_{F_{5}}^3}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_2p_1p_2*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{1}QS_{12}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{1}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_4p_1*}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1*}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_4p_1*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1*}}}{{M_{F_{5}}} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH2}} =
 
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
+\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{2 {M_{F_{1}}^3}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{4 {M_{F_{5}}^3}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{9L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{9}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH2}^\dagger } =
 
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
+\frac{{y}_{{d}}^{{f_5f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{2 {M_{F_{1}}^3}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1*}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{{y}_{{d}}^{{f_5f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{4 {M_{F_{5}}^3}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_4p_1*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3*}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{F_{9L}LS_{12}^\dagger }}^{{p_2f_3p_1*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{9}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2*}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2*}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2*}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2*}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_2f_5p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_5p_2*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_2p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_5p_2*}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLueH}} =
 \frac{8 \mathcal{D}_{{dF_{12R}^\dagger V_{3}}}^{{f_1p_1p_2*}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}}}{{M_{F_{12}}} {M_{V_{3}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_2f_2p_1*}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_2f_5p_1*}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_4p_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{D}_{{F_{10R}^\dagger uV_{3}^\dagger }}^{{p_1f_5p_2}}}{{M_{F_{10}}} {M_{V_{3}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{12R}^\dagger S_{12}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}}}{{M_{F_{12}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{3L}S_{12}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{3}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{eF_{1}V_{2}}}^{{f_4p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_2f_2p_1*}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_1p_2}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLueH}^\dagger } =
 \frac{8 \mathcal{D}_{{dF_{12R}^\dagger V_{3}}}^{{f_4p_1p_2}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_5p_2}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}}}{{M_{F_{12}}} {M_{V_{3}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_2}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_2f_5p_1}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_2f_2p_1}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_1p_1p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_5p_2}} \mathcal{D}_{{F_{10R}^\dagger uV_{3}^\dagger }}^{{p_1f_2p_2*}}}{{M_{F_{10}}} {M_{V_{3}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_2f_2}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_5p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_4p_1p_2*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_2f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_4p_1p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{e^\dagger F_{12R}^\dagger S_{12}}}^{{f_1p_2p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_2}}}{{M_{F_{12}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{3L}S_{12}u^\dagger }}^{{p_2p_1f_2}}}{{M_{F_{3}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_2f_2}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_2p_1*}} \mathcal{D}_{{eF_{1}V_{2}}}^{{f_1p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_2p_1*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_2f_5p_1}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_2p_1*}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_5p_2}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_1p_2*}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{QuLLH}} =
 \frac{{y}_{{u}}^{{f_4f_5}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{2 {M_{F_{1}}^3}}
+\frac{8 \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{{y}_{{u}}^{{f_4f_5}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}^3}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_2}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_2}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_2}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_2}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
+\frac{32 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_1*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
-\frac{16 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_1*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{32 \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{QuLLH}^\dagger } =
 \frac{{y}_{{u}}^{{f_2f_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}}}{2 {M_{F_{1}}^3}}
+\frac{{y}_{{u}}^{{f_2f_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}}}{4 {M_{F_{5}}^3}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_2*}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_2*}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_2*}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_2*}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_1f_4p_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_5p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_4f_1p_2}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_2p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_4f_1p_2}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_2}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_4p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_2p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
-\frac{16 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_4f_2p_1}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_5p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_4f_2p_2}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_4f_2p_2}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_5p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_4f_2p_2}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{32 \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_4f_2p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{32 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_4f_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_1}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_1f_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_5f_2p_2}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_5p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_5f_4p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_4p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_5p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_5f_4p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_2f_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdudH}} =
 \frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_2*}} \mathcal{D}_{{F_{10R}^\dagger S_{12}^\dagger u^\dagger }}^{{p_1p_2f_5*}}}{{M_{F_{10}}} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_4p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_2*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_2p_1p_2*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdudH}^\dagger } =
 
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_4}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_3p_1}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_4}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_3p_1}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_4}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_2f_4}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_4}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_2f_4}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_2p_1p_2}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_2f_4}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_2f_4}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{10R}^\dagger S_{12}^\dagger u^\dagger }}^{{p_1p_2f_4}}}{{M_{F_{10}}} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_2f_4}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_3p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_4}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_2p_1p_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_2f_4}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_3p_1}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_2f_4}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdddH}} =
 
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_5p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_5p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}}}{{M_{F_{11}}} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdddH}^\dagger } =
 \frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_1p_2p_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_4}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_1p_2p_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_4}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_3f_4p_2}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_4p_2}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_4p_2}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_3p_1p_2}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_4p_2}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_3p_1}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_2p_1p_2}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_4p_2}}}{{M_{F_{11}}} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eQddH}} =
 \frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_5f_1p_1*}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_5p_1*}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_1p_1p_2*}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_5p_1p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{3L}QS_{11}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{3}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger F_{8L}S_{11}^\dagger }}^{{f_1p_2p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_5p_2*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_2f_2p_1*}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_5p_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_5p_1p_2*}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eQddH}^\dagger } =
 \frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_2f_5p_2*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_2f_5p_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_4p_1p_2}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_2f_5p_2*}} \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{3L}QS_{11}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{3}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{8L}S_{11}^\dagger }}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{8}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_4f_5p_2*}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_2f_4p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_2}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_2f_5p_1}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_2f_4p_1}} \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_1p_2p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_4f_5p_2*}}}{{M_{F_{10}}} {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdQQH}} =
 
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_2p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_1p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_1p_1}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_1p_1}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{8L}QS_{12}}}^{{p_2f_1p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{S_{12}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_2p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_4p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_4p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
+\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdQQH}^\dagger } =
 
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_1f_5p_1*}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_5p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_4p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_1f_5p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_4p_1*}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_4p_1*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_5p_1*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_1f_5p_1*}} \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_2f_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{8L}QS_{12}}}^{{p_2f_5p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{8}}} {M_{S_{12}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_2f_5p_2*}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_2f_5p_2*}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_2p_1}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_2f_5p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_5p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_1p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_1f_5p_1*}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_5p_2*}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_1p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_5p_2*}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_5p_2*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_5p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_5p_2*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_5p_2*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{QQS_{10}}}^{{f_5f_4p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{QQS_{10}}}^{{f_5f_4p_2*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_5f_4p_2*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_5p_2*}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
+\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_5p_2*}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_5p_2*}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{QQS_{14}}}^{{f_5f_4p_2*}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{QQS_{14}}}^{{f_5f_4p_2*}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}} \mathcal{D}_{{QQS_{14}}}^{{f_5f_4p_2*}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}


==> result/eftdim7_unren.tex <==
\begin{align}
\begin{autobreak}
 {O_{5}} =
 
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mu_H^2 }{2 {M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mu_H^2 }{4 {M_{F_{5}}^3}}
-\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{2 {M_{F_{1}}}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi }} =
 \frac{2 \lambda_H (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}}}{{M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}}}{3 {M_{S_{7}}^2}}
+\frac{\mathcal{E}_{{HHHH^\dagger S_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{HHHH^\dagger S_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
+\frac{4 \lambda_H \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{4 \lambda_H \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}}}{{M_{V_{15}}^2}}
-\frac{8 \lambda_H \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{E}_{{HHH^\dagger H^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{1}S_{1}}}^{{p_1p_2}}}{{M_{S_{1}}^4}}
+\frac{\mathcal{E}_{{HHH^\dagger H^\dagger S_{5}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{HH^\dagger S_{1}S_{5}}}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(1)}}^{{p_2p_1}}}{4 {M_{S_{5}}^4}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{5}S_{5}(2)}}^{{p_2p_1}}}{2 {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_2p_1}}}{{M_{S_{6}}^4}}
+\frac{8 \lambda_H \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}}}{{M_{S_{1}}^4} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_2*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1*}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_1}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}}}{3 {M_{S_{5}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1*}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_3}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3*}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1*}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_3}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_1}}}{4 {M_{S_{4}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_3p_1*}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_3p_2}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{1}S_{1}}}^{{p_1p_2p_3}}}{{M_{S_{1}}^6}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{5}S_{5}}}^{{p_1p_3p_2}}}{2 {M_{S_{1}}^2} {M_{S_{5}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_3p_2p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi box}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}})^2}{2 {M_{S_{1}}^4}}
+\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{4 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi D}} =
 
-\frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{2 (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}}}{{M_{V_{15}}^2}}
+\frac{4 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}}}{{M_{V_{2}}^2}}
-\frac{4 \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{e\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{e}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{e}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{p_1p_2}}}{2 {M_{F_{3}}^2}}
+\frac{{y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_2*}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{p_1p_2}}}{2 {M_{F_{4}}^2}}
-\frac{\mathcal{E}_{{e^\dagger F_{2R}^\dagger HH^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_5*}}}{{M_{F_{2}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2p_1}}}{2 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{3L}H}}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{3}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{2R}^\dagger F_{4L}H^\dagger }}^{{p_2p_1*}}}{{M_{F_{2}}} {M_{F_{4}}}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{E}_{{F_{3L}HH^\dagger L(2)}}^{{p_1f_5*}}}{{M_{F_{3}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{E}_{{F_{4L}H^\dagger H^\dagger L(1)}}^{{p_1f_5*}}}{{M_{F_{4}}}}
-\frac{\mathcal{E}_{{e^\dagger F_{5}H^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}}}{{M_{F_{5}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}}}{{M_{F_{3}}} {M_{F_{5}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{2 {M_{F_{5}}^2}}
-\frac{\mathcal{E}_{{e^\dagger F_{6R}^\dagger HH^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}}}{2 {M_{F_{6}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}F_{6R}^\dagger H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}}}{2 {M_{F_{4}}} {M_{F_{6}}}}
+\frac{{y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_5*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1}}}{4 {M_{F_{6}}^2}}
-\frac{\mathcal{E}_{{e^\dagger HLS_{6}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{E}_{{e^\dagger H^\dagger LS_{1}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{2R}^\dagger S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{2}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{E}_{{e^\dagger H^\dagger LS_{5}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{2 {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{6R}^\dagger S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{6}}} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{f_5p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {y}_{{e}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{p_1f_5p_2}}}{2 {M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{u\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{S_{5}}^4}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{u}}^{{f_4f_5}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{u}}^{{f_4f_5}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2p_1}}}{{M_{F_{11}}^2}}
-\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{E}_{{F_{11R}^\dagger HH^\dagger Q(1)}}^{{p_1f_4*}}}{{M_{F_{11}}}}
+\frac{2 {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2p_1}}}{{M_{F_{12}}^2}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{E}_{{F_{12R}^\dagger HHQ(1)}}^{{p_1f_4*}}}{{M_{F_{12}}}}
-\frac{4 \mathcal{E}_{{F_{13L}HHu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{13}}}}
-\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_4*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{2 \mathcal{E}_{{F_{14L}HH^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{14}}}}
+\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{14L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{14}}}}
+\frac{{y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
-\frac{4 \mathcal{E}_{{F_{9L}HH^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}}}
+\frac{8 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger F_{9L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{11}}} {M_{F_{9}}}}
-\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger F_{9L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}}}{{M_{F_{12}}} {M_{F_{9}}}}
+\frac{2 {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{9}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2*}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{4 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{F_{9L}S_{1}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{9}}} {M_{S_{1}}^2}}
+\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_4p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
+\frac{2 \mathcal{D}_{{F_{14L}S_{5}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{14}}} {M_{S_{5}}^2}}
+\frac{2 \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{HQS_{1}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{1}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{E}_{{HQS_{5}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{5}}^2}}
+\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{E}_{{H^\dagger QS_{6}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{6}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_4p_2}}}{{M_{V_{1}}^2}}
+\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
-\frac{i {y}_{{u}}^{{p_1f_5}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_4p_2}}}{{M_{V_{4}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{u}}^{{f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{d\phi }} =
 \frac{(\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{S_{5}}^4}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{{M_{V_{1}}^2}}
-\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{(\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2 {y}_{{d}}^{{f_5f_4}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{15}}^2}}
-\frac{2 \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{2}}^2}}
+\frac{2 \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}} {y}_{{d}}^{{f_5f_4}}}{{M_{V_{4}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{p_1p_2}}}{{M_{F_{10}}^2}}
+\frac{2 {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{p_1p_2}}}{{M_{F_{11}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{E}_{{F_{10R}^\dagger H^\dagger H^\dagger Q(1)}}^{{p_1f_5*}}}{{M_{F_{10}}}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{E}_{{F_{11R}^\dagger HH^\dagger Q(2)}}^{{p_1f_5*}}}{{M_{F_{11}}}}
-\frac{2 \mathcal{E}_{{d^\dagger F_{13L}HH^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_5*}}}{{M_{F_{13}}}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{13L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{13}}}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{13L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{13}}}}
+\frac{{y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{13}}^2}}
+\frac{4 \mathcal{E}_{{d^\dagger F_{14L}H^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}}}{{M_{F_{14}}}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{14L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{14}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_5*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2p_1}}}{{M_{F_{14}}^2}}
-\frac{4 \mathcal{E}_{{d^\dagger F_{8L}HH^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_5*}}}{{M_{F_{8}}}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger F_{8L}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{10}}} {M_{F_{8}}}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger F_{8L}H}}^{{p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}}}{{M_{F_{11}}} {M_{F_{8}}}}
+\frac{2 {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2p_1}}}{{M_{F_{8}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HQS_{6}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_5p_2*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_5*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{E}_{{d^\dagger H^\dagger QS_{1}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{1}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{8L}S_{1}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{8}}} {M_{S_{1}}^2}}
+\frac{\mathcal{E}_{{d^\dagger H^\dagger QS_{5}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{{M_{S_{5}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11R}^\dagger QS_{5}}}^{{p_1f_5p_2*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{11}}} {M_{S_{5}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{13L}S_{5}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_5*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{{M_{F_{13}}} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{f_5p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{p_1f_4p_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_4f_5p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_1p_2*}}}{{M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
+\frac{2 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{p_1f_5p_2}}}{{M_{V_{1}}^2}}
-\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}}
+\frac{i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{p_1f_5p_2}}}{{M_{V_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi G}} =
 \frac{4 \mathcal{E}_{{GLGLS_{1}}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
+\frac{4 \mathcal{E}_{{GLGLS_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi Gt}} =
 \frac{4 i \mathcal{E}_{{GLGLS_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
-\frac{4 i \mathcal{E}_{{GLGLS_{1}}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi W}} =
 
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{S_{1}WLWL}}^{{p_1*}}}{{M_{S_{1}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{S_{1}WLWL}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi Wt}} =
 \frac{i \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{S_{1}WLWL}}^{{p_1*}}}{{M_{S_{1}}^2}}
-\frac{i \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{S_{1}WLWL}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi B}} =
 \frac{\mathcal{E}_{{BLBLS_{1}}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
+\frac{\mathcal{E}_{{BLBLS_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi Bt}} =
 \frac{i \mathcal{E}_{{BLBLS_{1}}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}}
-\frac{i \mathcal{E}_{{BLBLS_{1}}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}}}{{M_{S_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi WB}} =
 \frac{\mathcal{E}_{{BLS_{5}WL}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{\sqrt{2} {M_{S_{5}}^2}}
-\frac{\mathcal{E}_{{BLS_{5}WL}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{3 \sqrt{2} {M_{S_{5}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi WtB}} =
 \frac{i \mathcal{E}_{{BLS_{5}WL}}^{{p_1*}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{3 \sqrt{2} {M_{S_{5}}^2}}
+\frac{i \mathcal{E}_{{BLS_{5}WL}}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}}}{\sqrt{2} {M_{S_{5}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eW}} =
 \frac{i \mathcal{E}_{{e^\dagger F_{6R}^\dagger WL}}^{{f_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_3*}}}{6 \sqrt{2} {M_{F_{6}}}}
-\frac{i \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_2p_1*}} \mathcal{E}_{{F_{3L}LWL}}^{{p_1f_3*}}}{6 \sqrt{2} {M_{F_{3}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eB}} =
 \frac{i \mathcal{E}_{{BLe^\dagger F_{2R}^\dagger }}^{{f_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_3*}}}{2 {M_{F_{2}}}}
-\frac{i \mathcal{E}_{{BLF_{3L}L}}^{{p_1f_3*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_2p_1*}}}{2 {M_{F_{3}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{uG}} =
 \frac{2 i \sqrt{2} \mathcal{E}_{{F_{9L}GLu^\dagger }}^{{p_1f_3*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_2*}}}{{M_{F_{9}}}}
-\frac{4 i \sqrt{2} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_3*}} \mathcal{E}_{{F_{11R}^\dagger GLQ}}^{{p_1f_2*}}}{{M_{F_{11}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{uW}} =
 \frac{i \sqrt{2} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_3*}} \mathcal{E}_{{F_{11R}^\dagger QWL}}^{{p_1f_2*}}}{3 {M_{F_{11}}}}
-\frac{i \sqrt{2} \mathcal{E}_{{F_{14L}u^\dagger WL}}^{{p_1f_3*}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_2*}}}{3 {M_{F_{14}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{uB}} =
 \frac{2 i \mathcal{E}_{{BLF_{11R}^\dagger Q}}^{{p_1f_2*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_3*}}}{{M_{F_{11}}}}
-\frac{2 i \mathcal{E}_{{BLF_{9L}u^\dagger }}^{{p_1f_3*}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_2*}}}{{M_{F_{9}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dG}} =
 \frac{4 i \sqrt{2} \mathcal{E}_{{d^\dagger F_{8L}GL}}^{{f_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_3*}}}{{M_{F_{8}}}}
-\frac{4 i \sqrt{2} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1*}} \mathcal{E}_{{F_{11R}^\dagger GLQ}}^{{p_1f_3*}}}{{M_{F_{11}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dW}} =
 \frac{i \sqrt{2} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1*}} \mathcal{E}_{{F_{11R}^\dagger QWL}}^{{p_1f_3*}}}{3 {M_{F_{11}}}}
+\frac{i \sqrt{2} \mathcal{E}_{{d^\dagger F_{13L}WL}}^{{f_2p_1*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_3*}}}{3 {M_{F_{13}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dB}} =
 \frac{2 i \mathcal{E}_{{BLd^\dagger F_{8L}}}^{{f_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_3*}}}{{M_{F_{8}}}}
+\frac{2 i \mathcal{E}_{{BLF_{11R}^\dagger Q}}^{{p_1f_3*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1*}}}{{M_{F_{11}}}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi l1}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{i \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
-\frac{3 \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi l3}} =
 
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{2 {M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{4 {M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_1f_4*}}}{4 {M_{F_{2}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4*}}}{8 {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_4*}}}{8 {M_{F_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi e}} =
 \frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{i \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}}}{2 {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_4p_1*}}}{2 {M_{F_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi q1}} =
 
-\frac{3 \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{3 \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
+\frac{2 i \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
+\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi q3}} =
 \frac{\mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{2 {M_{F_{13}}^2}}
+\frac{\mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4*}}}{2 {M_{F_{14}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{i \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}}}{{M_{F_{8}}^2}}
-\frac{\mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4*}}}{{M_{F_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi u}} =
 
-\frac{2 \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_4*}}}{{M_{F_{11}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_4*}}}{{M_{F_{12}}^2}}
+\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi d}} =
 \frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}}}{{M_{V_{1}}^2}}
-\frac{2 i \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_4p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}}}{{M_{F_{10}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_1p_1}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}}}{{M_{F_{11}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{\phi ud}} =
 \frac{4 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_1}}}{{M_{F_{11}}^2}}
+\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_4f_1p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ll}} =
 
-\frac{\mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}}
+\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_4p_1}}}{4 {M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_4p_1}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_2f_3p_1}}}{2 {M_{V_{4}}^2}}
+\frac{\mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_1*}}}{2 {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_1*}}}{4 {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qq1}} =
 \frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
-\frac{2 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{3 \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
+\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{3 \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qq3}} =
 
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_4p_1}}}{3 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{\mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_1f_4p_1}} \mathcal{D}_{{QQ^\dagger V_{14}}}^{{f_2f_3p_1}}}{2 {M_{V_{14}}^2}}
-\frac{\mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_4f_3p_1*}}}{4 {M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_4f_3p_1*}}}{8 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{\mathcal{D}_{{QQS_{18}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{QQS_{18}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{18}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lq1}} =
 \frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{3 \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{3 \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lq3}} =
 
-\frac{\mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{4}}}^{{f_2f_4p_1}}}{{M_{V_{4}}^2}}
-\frac{2 \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{5}}^2}}
+\frac{\mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ee}} =
 \frac{\mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger e^\dagger S_{3}^\dagger }}^{{f_4f_3p_1*}}}{2 {M_{S_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{2 {M_{V_{1}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{uu}} =
 
-\frac{2 \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
+\frac{4 \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{17}u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{17}}^2}}
-\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_1f_2}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_2f_1}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dd}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_4p_1}}}{3 {M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_2f_3p_1}}}{{M_{V_{12}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}}}{{M_{S_{11}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_2f_1p_1}} \mathcal{D}_{{d^\dagger d^\dagger S_{15}}}^{{f_4f_3p_1*}}}{{M_{S_{15}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eu}} =
 
-\frac{4 \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_1f_4p_1*}} \mathcal{D}_{{eu^\dagger V_{6}}}^{{f_3f_2p_1}}}{{M_{V_{6}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ed}} =
 
-\frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_3f_2p_1*}}}{{M_{V_{5}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_3f_4p_1*}}}{{M_{S_{9}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ud1}} =
 
-\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{16}}^2}}
-\frac{128 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{9 {M_{V_{13}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ud8}} =
 
-\frac{32 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{13}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{13}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{le}} =
 \frac{\mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{2 {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lu}} =
 \frac{2 \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{4 \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ld}} =
 \frac{2 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_3f_4p_1*}}}{{M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qe}} =
 \frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger eV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qu1}} =
 \frac{4 \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
+\frac{32 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{V_{11}}^2}}
+\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{3 {M_{V_{7}}^2}}
-\frac{16 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qu8}} =
 \frac{16 \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{u^\dagger uV_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{11}^\dagger }}^{{f_3f_2p_1*}}}{{M_{V_{11}}^2}}
-\frac{2 \mathcal{D}_{{QuV_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_3f_2p_1*}}}{{M_{V_{7}}^2}}
+\frac{4 \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_3p_1f_4*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_1p_1f_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qd1}} =
 \frac{32 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{3 {M_{V_{10}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{3 {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger dV_{1}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{1}}}^{{f_2f_4p_1}}}{{M_{V_{1}}^2}}
-\frac{64 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{9 {M_{S_{19}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qd8}} =
 \frac{16 \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{10}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{10}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_1f_4p_1*}} \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}}}{{M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger dV_{12}}}^{{f_1f_3p_1}} \mathcal{D}_{{QQ^\dagger V_{12}}}^{{f_2f_4p_1}}}{{M_{V_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_3f_4p_1*}}}{3 {M_{S_{19}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{ledq}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_3p_1}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4f_2p_1}}}{{M_{V_{5}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_1f_4p_1}} \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_2p_1}}}{{M_{V_{7}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_3f_4p_1*}}}{{M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd1}} =
 \frac{4 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{3 {M_{S_{10}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{3 {M_{S_{16}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{3 {M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{quqd8}} =
 \frac{16 \mathcal{D}_{{d^\dagger QS_{19}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{QS_{19}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{19}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1*}}}{{M_{S_{10}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{16}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger S_{16}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{QQS_{16}^\dagger }}^{{f_3f_2p_1*}}}{{M_{S_{16}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ1}} =
 
-\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1*}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_3p_1f_4*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{13}}^2}}
-\frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{lequ3}} =
 \frac{\mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_1p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_2f_3p_1*}}}{2 {M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_2p_1f_4*}}}{2 {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duq}} =
 
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_3f_2p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_4p_1*}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger L^\dagger V_{7}}}^{{f_3f_1p_1*}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqu}} =
 \frac{2 \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_3p_1f_4*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{eQV_{7}^\dagger }}^{{f_3f_1p_1}} \mathcal{D}_{{QuV_{7}}}^{{f_2f_4p_1}}}{{M_{V_{7}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{qqq}} =
 \frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_3p_1}}}{{M_{S_{10}}^2}}
+\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_3p_1}}}{{M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{10}}}^{{f_3f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{\mathcal{D}_{{LQS_{14}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{QQS_{14}}}^{{f_3f_2p_1}}}{{M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duu}} =
 
-\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_3f_4*}}}{{M_{S_{9}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger e^\dagger S_{9}}}^{{f_1f_2p_1*}} \mathcal{D}_{{S_{9}^\dagger u^\dagger u^\dagger }}^{{p_1f_4f_3*}}}{{M_{S_{9}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_1p_1f_3*}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_2p_1f_4*}}}{{M_{S_{10}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LH}} =
 
-\frac{{C}_5^{{f_1f_2}} (\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}})^2}{{M_{S_{5}}^4}}
+\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1*}})^2}{{M_{V_{1}}^2}}
-\frac{2 {C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_1}})^2}{{M_{V_{1}}^2}}
+\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}})^2}{{M_{V_{4}}^2}}
-\frac{{C}_5^{{f_1f_2}} (\mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}})^2}{{M_{V_{4}}^2}}
+\frac{\lambda_H \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}^3}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{2 {M_{F_{1}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{2 {M_{F_{1}}^2}}
-\frac{\mathcal{E}_{{F_{1}F_{1}HH^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}}}{{M_{F_{1}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_3p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_3f_1}}}{{M_{F_{1}}^2} {M_{F_{3}}}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_2f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_2f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}}}
-\frac{\mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_1f_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}}}{{M_{F_{3}}}}
+\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_2f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}}}
+\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_2f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}}}
+\frac{\lambda_H \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{2 {M_{F_{5}}^3}}
+\frac{\mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_1f_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{5}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{4 {M_{F_{5}}^2}}
-\frac{\mathcal{E}_{{F_{1}F_{5}HH^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{2 {M_{F_{1}}} {M_{F_{5}}}}
+\frac{\mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_1f_1}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{4 {M_{F_{3}}} {M_{F_{5}}}}
-\frac{3 \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{4 {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{E}_{{F_{5}F_{5}HH^\dagger (1)}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{2 {M_{F_{5}}^2}}
+\frac{\mathcal{E}_{{F_{5}F_{5}HH^\dagger (2)}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{4 {M_{F_{5}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_3p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{3 {M_{F_{5}}^2} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}}}{{M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{E}_{{F_{1}F_{6R}^\dagger HH}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{2 {M_{F_{1}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{{M_{F_{3}}} {M_{F_{6}}}}
-\frac{\mathcal{E}_{{F_{5}F_{6R}^\dagger HH(2)}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{4 {M_{F_{5}}} {M_{F_{6}}}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
-\frac{{C}_5^{{f_2p_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{2 {M_{F_{6}}^2}}
-\frac{{C}_5^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2p_1*}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}}}{2 {M_{F_{6}}^2}}
-\frac{3 \mathcal{E}_{{F_{1}F_{6R}^\dagger HH}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{2 {M_{F_{1}}} {M_{F_{6}}}}
-\frac{2 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{{M_{F_{3}}} {M_{F_{6}}}}
+\frac{3 \mathcal{E}_{{F_{5}F_{6R}^\dagger HH(2)}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{4 {M_{F_{5}}} {M_{F_{6}}}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{F_{6}}}}
-\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_1}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
+\frac{5 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_2}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{F_{6}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_1}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_3f_2}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_3p_2}}}{2 {M_{F_{5}}} {M_{F_{6}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{7L}HH^\dagger L}}^{{p_2f_1}}}{6 {M_{F_{5}}} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{7L}HH^\dagger L}}^{{p_2f_2}}}{2 {M_{F_{5}}} {M_{F_{7}}}}
+\frac{\mathcal{E}_{{F_{7L}HH^\dagger L}}^{{p_1f_2}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_1f_1}}}{3 {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_2f_1}}}{6 {M_{F_{5}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_1p_2}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_2f_1}}}{3 {M_{F_{6}}} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_2f_2}}}{6 {M_{F_{5}}} {M_{F_{7}}}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_1p_2}} \mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_2}}}{{M_{F_{6}}} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_2}}}{6 {M_{F_{5}}} {M_{S_{7}}^2}}
-\frac{2 {C}_5^{{f_1f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{1}H^\dagger LS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{1}H^\dagger LS_{6}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{F_{3L}HH^\dagger L(1)}}^{{p_1f_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{5}H^\dagger LS_{6}(1)}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{5}H^\dagger LS_{6}(1)}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{5}H^\dagger LS_{6}(2)}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{5}H^\dagger LS_{6}(2)}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{E}_{{F_{6R}^\dagger HLS_{6}(2)}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{F_{7L}HH^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{3 {M_{F_{7}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_2f_2p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{F_{1}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{3L}F_{6R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{{M_{F_{3}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{3 \mathcal{D}_{{F_{5}F_{6R}^\dagger S_{6}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_2f_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{4 {M_{F_{5}}} {M_{F_{6}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger F_{7L}H}}^{{p_1p_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{3 {M_{F_{6}}} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7L}H^\dagger }}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_2f_2p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{2 {C}_5^{{f_1f_2}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{15}^\dagger D}}^{{p_1}}}{{M_{V_{15}}^2}}
+\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_2*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{1}HLS_{1}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{1}HLS_{1}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{5}HLS_{1}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{5}HLS_{1}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{1}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}}}{{M_{F_{3}}} {M_{S_{1}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{1}S_{1}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{{M_{F_{1}}^2} {M_{S_{1}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}LS_{1}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{5}S_{1}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}}}{2 {M_{F_{5}}^2} {M_{S_{1}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{1}HLS_{5}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{4 {M_{F_{1}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{1}HLS_{5}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{4 {M_{F_{1}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_1p_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_3}} \mathcal{D}_{{F_{5}HL}}^{{p_3f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{3}}} {M_{F_{5}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{5}HLS_{5}(1)}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{5}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{5}HLS_{5}(1)}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{5}HLS_{5}(2)}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{E}_{{F_{5}HLS_{5}(2)}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{8 {M_{F_{5}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{7L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_1f_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{3 {M_{F_{7}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{3L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{7L}LS_{5}}}^{{p_1f_2p_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_1p_3}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}}}{3 {M_{F_{7}}} {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{3 \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{3L}LS_{5}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{4 {M_{F_{1}}} {M_{F_{3}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}F_{5}S_{5}}}^{{p_1p_2p_3}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{1}}} {M_{F_{5}}} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_1p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{6 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{7L}LS_{5}}}^{{p_2f_2p_3}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}}}{2 {M_{F_{5}}} {M_{F_{7}}} {M_{S_{5}}^2}}
-\frac{4 {C}_5^{{f_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1*}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_1}}}{{M_{V_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_1f_2p_1}}}{{M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_1f_2p_1}}}{{M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{E}_{{HLLS_{7}}}^{{f_1f_2p_1}}}{3 {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2}}}{{M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{2 {M_{F_{1}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_3}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_3p_2}}}{4 {M_{F_{5}}} {M_{S_{1}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{2 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3*}}}{4 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{E}_{{HLLS_{7}}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_2}}}{3 {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_3p_2}}}{6 {M_{F_{5}}} {M_{S_{5}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{6L}H^\dagger L}}^{{p_1f_2}} \mathcal{D}_{{F_{6R}^\dagger LS_{8}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_3p_2}}}{{M_{F_{6}}} {M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{E}_{{HLLS_{7}}}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_2*}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{7}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_3}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2*}}}{6 {M_{F_{5}}} {M_{S_{6}}^2} {M_{S_{7}}^2}}
+\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{E}_{{H^\dagger LLS_{8}}}^{{f_1f_2p_1}}}{{M_{S_{8}}^2}}
+\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_2}} \mathcal{E}_{{H^\dagger LLS_{8}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_1f_2p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_1f_2p_2}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1*}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
+\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{4 {M_{F_{1}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_3*}}}{8 {M_{F_{5}}} {M_{S_{4}}^2} {M_{S_{5}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{E}_{{LLS_{1}S_{6}}}^{{f_1f_2p_2p_1}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{E}_{{LLS_{5}S_{6}(1)}}^{{f_1f_2p_2p_1}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{E}_{{HHHH^\dagger S_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}}}{{M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HHS_{1}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{1}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{HHS_{5}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{HH^\dagger S_{6}S_{6}^\dagger (2)}}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^4}}
+\frac{\mathcal{D}_{{HH^\dagger H^\dagger S_{4}(1)}}^{{p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{HHHS_{8}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^2} {M_{S_{8}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_2p_3*}} \mathcal{C}_{{HS_{6}S_{8}^\dagger }}^{{p_1p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{S_{6}}^4} {M_{S_{8}}^2}}
-\frac{\mathcal{D}_{{HHH^\dagger S_{7}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{3 {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HH^\dagger S_{1}}}^{{p_1}} \mathcal{C}_{{HS_{1}S_{4}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{{M_{S_{1}}^2} {M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_1*}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{{M_{S_{4}}^2} {M_{S_{6}}^4}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{5}S_{7}^\dagger }}^{{p_1p_2}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{3 {M_{S_{5}}^2} {M_{S_{6}}^2} {M_{S_{7}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_1p_2*}} \mathcal{C}_{{HS_{6}^\dagger S_{7}}}^{{p_3p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{3 {M_{S_{6}}^4} {M_{S_{7}}^2}}
+\frac{\mathcal{C}_{{HH^\dagger S_{5}}}^{{p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_2p_3}} \mathcal{C}_{{H^\dagger S_{4}S_{5}}}^{{p_2p_1*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}}}{2 {M_{S_{4}}^2} {M_{S_{5}}^2} {M_{S_{6}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{1}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{1}}}^{{f_1p_1p_2}}}{{M_{V_{1}}^2}}
+\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
+\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2*}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {C}_5^{{f_2p_1}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{i {C}_5^{{p_1f_2}} \mathcal{D}_{{HH^\dagger V_{4}D}}^{{p_2}} \mathcal{D}_{{LL^\dagger V_{4}}}^{{f_1p_1p_2}}}{2 {M_{V_{4}}^2}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{1}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}} \mathcal{C}_{{S_{1}S_{6}S_{6}^\dagger }}^{{p_2p_1p_3}}}{{M_{S_{1}}^2} {M_{S_{6}}^4}}
-\frac{\mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{C}_{{HH^\dagger S_{5}}}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_3}} \mathcal{C}_{{S_{5}S_{6}S_{6}^\dagger }}^{{p_2p_1p_3}}}{2 {M_{S_{5}}^2} {M_{S_{6}}^4}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LeHD}} =
 
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^3}}
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{LLS_{6}}}^{{f_1p_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{S_{6}}^4}}
-\frac{2 {y}_{{e}}^{{p_1f_5}} \mathcal{E}_{{LLV_{2}D}}^{{f_1p_1p_2}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}}}{{M_{V_{2}}^2}}
-\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^3}}
+\frac{{y}_{{e}}^{{p_1f_5}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_1p_2}}}{{M_{S_{6}}^4}}
-\frac{2 {y}_{{e}}^{{p_1f_5}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{E}_{{LLV_{2}D}}^{{p_1f_1p_2}}}{{M_{V_{2}}^2}}
+\frac{2 i \mathcal{D}_{{eF_{1}V_{2}}}^{{f_5p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
-\frac{2 i \mathcal{E}_{{eHLV_{2}}}^{{f_5f_1p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_1}}}{{M_{F_{1}}} {M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3L}F_{5}H^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{{M_{F_{3}}} {M_{F_{5}}^2}}
+\frac{2 i \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_1}}}{2 {M_{F_{3}}^2} {M_{F_{5}}}}
+\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_1}}}{{M_{F_{3}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_1p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{3}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{e^\dagger F_{5}H^\dagger H^\dagger }}^{{f_5p_1*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}}}{{M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_5p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{{M_{F_{5}}^2} {M_{S_{6}}^2}}
-\frac{2 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_5f_1p_1*}} \mathcal{E}_{{HHHV_{3}^\dagger D(1)}}^{{p_1}}}{{M_{V_{3}}^2}}
-\frac{2 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_5f_1p_1*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{HS_{6}V_{3}^\dagger D}}^{{p_2p_1}}}{{M_{S_{6}}^2} {M_{V_{3}}^2}}
-\frac{4 i \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_5f_1p_1*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_2p_1}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD1}} =
 \frac{2 \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{4 \mathcal{E}_{{LLV_{2}D}}^{{f_1f_2p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{{M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHD2}} =
 
-\frac{4 \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{\mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}^3}}
-\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{2 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHB}} =
 
-\frac{\mathcal{E}_{{BLF_{1}F_{1}}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}}}{2 {M_{F_{1}}^2}}
+\frac{\mathcal{E}_{{BLF_{3L}L}}^{{p_1f_2}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}}}{4 {M_{F_{1}}} {M_{F_{3}}}}
+\frac{3 \mathcal{E}_{{BLF_{3L}L}}^{{p_1f_3}} \mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}}}{4 {M_{F_{1}}} {M_{F_{3}}}}
-\frac{\mathcal{E}_{{BLF_{3L}L}}^{{p_1f_2}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}}}{8 {M_{F_{3}}} {M_{F_{5}}}}
+\frac{\mathcal{E}_{{BLF_{3L}L}}^{{p_1f_3}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{8 {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{E}_{{BLF_{3L}L}}^{{p_1f_3}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_2}}}{2 {M_{F_{3}}}}
+\frac{\mathcal{E}_{{BLF_{3L}L}}^{{p_1f_3}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{2 {M_{F_{3}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{BLF_{5}F_{5}}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}}}{4 {M_{F_{5}}^2}}
-\frac{i {g'} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{8 {M_{F_{1}}^3}}
-\frac{i {g'} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{2 {M_{S_{6}}^4}}
-\frac{i {g'} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{16 {M_{F_{5}}^3}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LHW}} =
 \frac{\mathcal{D}_{{F_{1}F_{3R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{3L}LWL}}^{{p_2f_3}}}{2 \sqrt{2} {M_{F_{1}}} {M_{F_{3}}}}
+\frac{\mathcal{E}_{{F_{1}F_{5}WL}}^{{p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}}}{2 \sqrt{2} {M_{F_{1}}} {M_{F_{5}}}}
+\frac{i {g} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_3}}}{8 {M_{F_{1}}^3}}
+\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{4 {M_{S_{6}}^4}}
-\frac{i {g} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{4 {M_{S_{6}}^4}}
+\frac{\mathcal{E}_{{F_{3L}LWL}}^{{p_1f_3}} \mathcal{D}_{{F_{3R}^\dagger F_{5}H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{4 \sqrt{2} {M_{F_{3}}} {M_{F_{5}}}}
-\frac{\mathcal{E}_{{F_{3L}LWL}}^{{p_1f_3}} \mathcal{E}_{{F_{3R}^\dagger HHL(1)}}^{{p_1f_2}}}{2 \sqrt{2} {M_{F_{3}}}}
+\frac{\mathcal{E}_{{F_{3L}LWL}}^{{p_1f_3}} \mathcal{D}_{{F_{3R}^\dagger LS_{6}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{2 \sqrt{2} {M_{F_{3}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{F_{5}F_{5}WL}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}}}{4 \sqrt{2} {M_{F_{5}}^2}}
+\frac{\mathcal{E}_{{F_{5}F_{5}WL}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}}}{4 \sqrt{2} {M_{F_{5}}^2}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{E}_{{F_{7L}LWL}}^{{p_2f_3}}}{6 \sqrt{2} {M_{F_{5}}} {M_{F_{7}}}}
+\frac{\mathcal{D}_{{F_{5}F_{7R}^\dagger H}}^{{p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}} \mathcal{E}_{{F_{7L}LWL}}^{{p_2f_2}}}{2 \sqrt{2} {M_{F_{5}}} {M_{F_{7}}}}
-\frac{3 i {g} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_3}}}{16 {M_{F_{5}}^3}}
+\frac{\mathcal{E}_{{F_{7L}LWL}}^{{p_1f_3}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_1f_2}}}{6 \sqrt{2} {M_{F_{7}}}}
+\frac{\mathcal{E}_{{F_{7L}LWL}}^{{p_1f_2}} \mathcal{E}_{{F_{7R}^\dagger HHL}}^{{p_1f_3}}}{2 \sqrt{2} {M_{F_{7}}}}
+\frac{\mathcal{E}_{{F_{7L}LWL}}^{{p_1f_2}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_3p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{2 \sqrt{2} {M_{F_{7}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{F_{7L}LWL}}^{{p_1f_3}} \mathcal{D}_{{F_{7R}^\dagger LS_{6}}}^{{p_1f_2p_2}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}}}{6 \sqrt{2} {M_{F_{7}}} {M_{S_{6}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{duLLD}} =
 
-\frac{8 i \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_1f_2p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3f_4p_1*}}}{{M_{V_{8}}^2}}
-\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{LLV_{2}D}}^{{f_2f_3p_1}}}{{M_{V_{2}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LQddD}} =
 \frac{4 i \mathcal{D}_{{dQV_{8}}}^{{f_2f_1p_1}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_3f_4p_1*}}}{{M_{V_{8}}^2}}
+\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_3f_2p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4f_1p_1}}}{{M_{V_{5}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{edddD}} =
 
-\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_4f_3p_1*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_2f_1p_1*}}}{{M_{V_{5}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eLLLH}} =
 \frac{{y}_{{e}}^{{f_1f_4*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}}}{{M_{S_{6}}^4}}
-\frac{2 {y}_{{e}}^{{f_1f_4*}} \mathcal{E}_{{LLV_{2}D}}^{{f_2f_3p_1}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}}}{{M_{V_{2}}^2}}
-\frac{{y}_{{e}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{2 {M_{F_{5}}^3}}
-\frac{{y}_{{e}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_3p_2}}}{{M_{S_{6}}^4}}
+\frac{2 {y}_{{e}}^{{p_1f_4*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{E}_{{LLV_{2}D}}^{{p_1f_3p_2}}}{{M_{V_{2}}^2}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{1}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2}}}{2 {M_{F_{1}}} {M_{S_{2}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{4L}LS_{2}^\dagger }}^{{p_1f_4p_2}}}{{M_{F_{4}}} {M_{S_{2}}^2}}
-\frac{\mathcal{D}_{{e^\dagger F_{4R}^\dagger H}}^{{f_1p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{4L}LS_{6}^\dagger }}^{{p_1f_4p_2}}}{2 {M_{F_{4}}} {M_{S_{6}}^2}}
-\frac{3 \mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_4}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_4p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger F_{5}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_4f_3p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{e^\dagger HLS_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_1}}}{{M_{S_{2}}^2}}
-\frac{\mathcal{E}_{{e^\dagger HLS_{6}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}}}{2 {M_{S_{6}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_4p_2}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_4f_3p_2}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_3p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_4}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_2f_3p_1}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}}}{2 {M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{\mathcal{D}_{{e^\dagger LS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{2 {M_{F_{5}}} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH1}} =
 \frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
-\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^3}}
-\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^3}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{1}}} {M_{S_{12}}^2}}
-\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^3}}
-\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^3}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_2f_3p_1}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_3f_2p_1}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_2f_3p_1}}}{{M_{S_{4}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_3f_2p_1}}}{{M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{E}_{{HLQS_{12}^\dagger (2)}}^{{f_3f_4p_1}}}{{M_{S_{12}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HQS_{6}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}}}{{M_{S_{6}}^2}}
+\frac{2 {y}_{{d}}^{{f_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}}}{{M_{S_{6}}^4}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HQS_{6}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}}}{{M_{S_{6}}^2}}
+\frac{2 {y}_{{d}}^{{f_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}}}{{M_{S_{6}}^4}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
-\frac{2 {y}_{{d}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_2p_2}}}{{M_{S_{6}}^4}}
-\frac{2 {y}_{{d}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_3p_2}}}{{M_{S_{6}}^4}}
-\frac{4 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HLS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1}}}{{M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLQLH2}} =
 
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{14L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{14}}} {M_{S_{12}}^2}}
+\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{1}HL}}^{{p_2p_1}}}{2 {M_{F_{1}}^3}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{2 {M_{F_{5}}^3}}
-\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}HL}}^{{p_2p_1}}}{4 {M_{F_{5}}^3}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_2f_3p_1}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_3}} \mathcal{D}_{{F_{5}QS_{12}^\dagger }}^{{p_2f_4p_1}}}{{M_{F_{5}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{F_{9L}LS_{12}^\dagger }}^{{p_2f_3p_1}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_2f_4}}}{{M_{F_{9}}} {M_{S_{12}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(1)}}^{{f_3f_2p_1}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{E}_{{HLLS_{4}(2)}}^{{f_2f_3p_1}}}{{M_{S_{4}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{E}_{{HLQS_{12}^\dagger (1)}}^{{f_3f_4p_1}}}{{M_{S_{12}}^2}}
+\frac{2 \mathcal{E}_{{d^\dagger HQS_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_1}}}{{M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_3p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HQS_{2}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_1}}}{{M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{2}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{9L}S_{2}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{9R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{F_{9}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_2p_1}} \mathcal{D}_{{LLS_{2}}}^{{f_3f_2p_2}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{\mathcal{E}_{{d^\dagger HQS_{6}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}}}{{M_{S_{6}}^2}}
-\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_1}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_3p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{E}_{{d^\dagger HQS_{6}^\dagger }}^{{f_1f_4p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}}}{{M_{S_{6}}^2}}
-\frac{{y}_{{d}}^{{f_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_1}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_1}}}{{M_{S_{6}}^4}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger QS_{6}^\dagger }}^{{p_1f_4p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{10}}} {M_{S_{6}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{14L}S_{6}^\dagger }}^{{f_1p_1p_2}} \mathcal{D}_{{F_{14R}^\dagger HQ}}^{{p_1f_4}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{F_{14}}} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{d^\dagger QS_{4}^\dagger }}^{{f_1f_4p_1}} \mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_3f_2p_2}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_2p_2}}}{{M_{S_{6}}^4}}
+\frac{{y}_{{d}}^{{p_1f_4*}} \mathcal{C}_{{HHS_{6}^\dagger }}^{{p_2}} \mathcal{D}_{{LLS_{6}}}^{{p_1f_3p_2}}}{{M_{S_{6}}^4}}
-\frac{2 {y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{E}_{{LLV_{2}D}}^{{f_2f_3p_1}}}{{M_{V_{2}}^2}}
+\frac{2 {y}_{{d}}^{{f_1f_4*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_1}} \mathcal{E}_{{LLV_{2}D}}^{{f_3f_2p_1}}}{{M_{V_{2}}^2}}
-\frac{2 {y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{E}_{{LLV_{2}D}}^{{p_1f_2p_2}}}{{M_{V_{2}}^2}}
+\frac{2 {y}_{{d}}^{{p_1f_4*}} \mathcal{D}_{{HHV_{2}^\dagger D}}^{{p_2}} \mathcal{E}_{{LLV_{2}D}}^{{p_1f_3p_2}}}{{M_{V_{2}}^2}}
+\frac{4 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_1}}}{{M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}} \mathcal{D}_{{LQS_{10}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{2 \mathcal{E}_{{d^\dagger HLS_{14}}}^{{f_1f_2p_1}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_1}}}{{M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_2p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_1p_1p_2}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2}} \mathcal{D}_{{LQS_{14}^\dagger }}^{{f_3f_4p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
-\frac{8 i {y}_{{u}}^{{p_1f_4*}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_1f_3p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2p_1p_2*}}}{{M_{V_{8}}^2}}
+\frac{8 i {y}_{{u}}^{{p_1f_4*}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_1f_2p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_3p_1p_2*}}}{{M_{V_{8}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{dLueH}} =
 \frac{8 \mathcal{D}_{{dF_{12R}^\dagger V_{3}}}^{{f_1p_1p_2*}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}}}{{M_{F_{12}}} {M_{V_{3}}^2}}
-\frac{4 \mathcal{E}_{{dH^\dagger u^\dagger V_{3}}}^{{f_1f_5p_1*}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_1*}}}{{M_{V_{3}}^2}}
+\frac{8 \mathcal{E}_{{d^\dagger eHV_{8}}}^{{f_1f_4p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_1*}}}{{M_{V_{8}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_2f_2p_1*}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}} \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_2f_5p_1*}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{E}_{{H^\dagger L^\dagger u^\dagger V_{5}}}^{{f_2f_5p_1*}}}{{M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_1f_4p_1}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_4p_1p_2}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{D}_{{F_{10R}^\dagger uV_{3}^\dagger }}^{{p_1f_5p_2}}}{{M_{F_{10}}} {M_{V_{3}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_1p_1}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_1p_1p_2}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{12R}^\dagger S_{12}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_2f_5*}}}{{M_{F_{12}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{3L}S_{12}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{3}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{E}_{{e^\dagger H^\dagger S_{12}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_1f_2p_1}} \mathcal{D}_{{e^\dagger S_{10}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_2}} {y}_{{e}}^{{p_1f_4}} \mathcal{E}_{{LLV_{2}D}}^{{f_2p_1p_2}}}{{M_{V_{2}}^2}}
+\frac{4 i \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_2}} {y}_{{e}}^{{p_1f_4}} \mathcal{E}_{{LLV_{2}D}}^{{p_1f_2p_2}}}{{M_{V_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{eF_{1}V_{2}}}^{{f_4p_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_2}}}{{M_{F_{1}}} {M_{V_{2}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{E}_{{eHLV_{2}}}^{{f_4f_2p_1}}}{{M_{V_{2}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{3L}L^\dagger V_{2}^\dagger }}^{{p_2f_2p_1*}}}{{M_{F_{3}}} {M_{V_{2}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger uV_{2}^\dagger }}^{{f_1f_5p_1}} \mathcal{D}_{{e^\dagger L^\dagger V_{3}^\dagger }}^{{f_4f_2p_2*}} \mathcal{C}_{{HV_{2}V_{3}^\dagger }}^{{p_1p_2}}}{{M_{V_{2}}^2} {M_{V_{3}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{QuLLH}} =
 \frac{{y}_{{u}}^{{f_4f_5}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{2 {M_{F_{1}}^3}}
+\frac{8 \mathcal{D}_{{F_{1}^\dagger u^\dagger V_{5}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{V_{5}}^2}}
+\frac{8 \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{F_{1L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_2}}}{{M_{F_{1}}} {M_{S_{4}}^2}}
+\frac{{y}_{{u}}^{{f_4f_5}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}}}{4 {M_{F_{5}}^3}}
+\frac{2 \mathcal{E}_{{H^\dagger QS_{2}u^\dagger }}^{{f_4p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}}}{{M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_2}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
-\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_2}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
-\frac{2 \mathcal{E}_{{H^\dagger QS_{2}u^\dagger }}^{{f_4p_1f_5*}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}}}{{M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{2}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_2}}}{{M_{F_{12}}} {M_{S_{2}}^2}}
+\frac{4 \mathcal{D}_{{F_{8L}S_{2}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_2}}}{{M_{F_{8}}} {M_{S_{2}}^2}}
-\frac{\mathcal{E}_{{H^\dagger QS_{6}u^\dagger }}^{{f_4p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_1}}}{{M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{\mathcal{E}_{{H^\dagger QS_{6}u^\dagger }}^{{f_4p_1f_5*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_1}}}{{M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger QS_{6}}}^{{p_1f_4p_2*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}}}{{M_{F_{12}}} {M_{S_{6}}^2}}
+\frac{2 \mathcal{D}_{{F_{13L}S_{6}u^\dagger }}^{{p_1p_2f_5*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}}}{{M_{F_{13}}} {M_{S_{6}}^2}}
-\frac{8 \mathcal{E}_{{H^\dagger L^\dagger u^\dagger V_{5}}}^{{f_2f_5p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}}}{{M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{5}}}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{12}}} {M_{V_{5}}^2}}
+\frac{4 \mathcal{E}_{{H^\dagger L^\dagger u^\dagger V_{9}}}^{{f_2f_5p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_1*}}}{{M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
-\frac{8 \mathcal{E}_{{H^\dagger L^\dagger u^\dagger V_{9}}}^{{f_1f_5p_1*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_1*}}}{{M_{V_{9}}^2}}
-\frac{16 \mathcal{D}_{{F_{12L}H^\dagger u^\dagger }}^{{p_1f_5*}} \mathcal{D}_{{F_{12R}^\dagger L^\dagger V_{9}}}^{{p_1f_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{12}}} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}^\dagger u^\dagger V_{9}}}^{{p_1f_5p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}}}{{M_{F_{5}}} {M_{V_{9}}^2}}
-\frac{8 \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (2)}}^{{f_2f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_1*}}}{{M_{V_{8}}^2}}
-\frac{8 \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (1)}}^{{f_2f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_1*}}}{{M_{V_{8}}^2}}
+\frac{32 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_2f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_1*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_1f_5p_2*}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (1)}}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_1*}}}{{M_{V_{8}}^2}}
-\frac{16 \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_1*}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{8 \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_4*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{32 \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_1f_4p_1*}} \mathcal{D}_{{L^\dagger u^\dagger V_{8}}}^{{f_2f_5p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
-\frac{2 \mathcal{E}_{{HLLS_{4}(1)}}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
-\frac{2 \mathcal{E}_{{HLLS_{4}(2)}}^{{f_2f_1p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_1f_2p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{C}_{{HS_{4}S_{6}^\dagger }}^{{p_1p_2}} \mathcal{D}_{{LLS_{6}}}^{{f_2f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{4}}^2} {M_{S_{6}}^2}}
+\frac{\mathcal{D}_{{F_{5}HL}}^{{p_1f_2}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_1p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{D}_{{F_{5}HL}}^{{p_1f_1}} \mathcal{D}_{{F_{5L}S_{4}}}^{{p_1f_2p_2}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{5}}} {M_{S_{4}}^2}}
-\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_1f_2p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}}
+\frac{2 \mathcal{C}_{{HS_{2}^\dagger S_{4}}}^{{p_1p_2}} \mathcal{D}_{{LLS_{2}}}^{{f_2f_1p_1}} \mathcal{D}_{{QS_{4}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{S_{2}}^2} {M_{S_{4}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdudH}} =
 
-\frac{4 i \mathcal{D}_{{dQV_{8}}}^{{f_3p_1p_2}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_2f_4p_2*}} {y}_{{u}}^{{p_1f_5}}}{{M_{V_{8}}^2}}
+\frac{8 \mathcal{E}_{{d^\dagger d^\dagger HS_{13}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{13}}^2}}
-\frac{8 \mathcal{E}_{{d^\dagger d^\dagger HS_{13}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{13}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_2f_5*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_4p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_4*}} \mathcal{D}_{{F_{1}S_{11}u^\dagger }}^{{p_2p_1f_5*}}}{{M_{F_{1}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{E}_{{HLS_{11}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{E}_{{HLS_{11}u^\dagger }}^{{f_4p_1f_5*}}}{{M_{S_{11}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
-\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_2f_3p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4p_1p_2}} {y}_{{u}}^{{p_1f_5}}}{{M_{V_{5}}^2}}
+\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_3f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_4p_1p_2}} {y}_{{u}}^{{p_1f_5}}}{{M_{V_{5}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{LS_{13}u^\dagger }}^{{f_4p_2f_5*}}}{{M_{F_{10}}} {M_{S_{13}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_2*}} \mathcal{D}_{{F_{10R}^\dagger S_{12}^\dagger u^\dagger }}^{{p_1p_2f_5*}}}{{M_{F_{10}}} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_4p_2*}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_2*}} \mathcal{D}_{{F_{11L}Hu^\dagger }}^{{p_1f_5*}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_2p_1p_2*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_4*}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{8 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_2f_4p_1*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_1f_5*}}}{{M_{S_{10}}^2}}
+\frac{8 \mathcal{E}_{{d^\dagger HS_{12}^\dagger u^\dagger }}^{{f_3p_1f_5*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}}}{{M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_4p_1*}} \mathcal{D}_{{d^\dagger S_{10}^\dagger u^\dagger }}^{{f_3p_2f_5*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdddH}} =
 \frac{4 i {y}_{{d}}^{{p_1f_4}} \mathcal{D}_{{dQV_{8}}}^{{f_3p_1p_2}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_2f_5p_2*}}}{{M_{V_{8}}^2}}
+\frac{16 i {y}_{{d}}^{{p_1f_4}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_2f_3p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5p_1p_2}}}{{M_{V_{5}}^2}}
-\frac{16 i {y}_{{d}}^{{p_1f_4}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_3f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5p_1p_2}}}{{M_{V_{5}}^2}}
-\frac{8 \mathcal{E}_{{d^\dagger d^\dagger H^\dagger S_{12}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}}}{{M_{S_{12}}^2}}
+\frac{8 \mathcal{E}_{{d^\dagger d^\dagger H^\dagger S_{12}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}}}{{M_{S_{12}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_5p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_4p_2*}} \mathcal{D}_{{F_{11R}^\dagger LS_{11}}}^{{p_2f_5p_1*}}}{{M_{F_{11}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger F_{2R}^\dagger S_{11}}}^{{f_4p_2p_1*}} \mathcal{D}_{{F_{2L}H^\dagger L}}^{{p_2f_5*}}}{{M_{F_{2}}} {M_{S_{11}}^2}}
+\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{E}_{{d^\dagger H^\dagger LS_{11}}}^{{f_4f_5p_1*}}}{{M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{E}_{{d^\dagger H^\dagger LS_{11}}}^{{f_4f_5p_1*}}}{{M_{S_{11}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_2f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_4f_3p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_2f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_3f_2p_1*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}} \mathcal{C}_{{HS_{11}^\dagger S_{12}}}^{{p_1p_2}}}{{M_{S_{11}}^2} {M_{S_{12}}^2}}
+\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_4f_3p_2*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_2p_1p_2*}} {y}_{{e}}^{{f_5p_1}}}{{M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_2p_1*}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_3p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}}}{{M_{F_{11}}} {M_{S_{12}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{11L}H^\dagger }}^{{f_3p_1*}} \mathcal{D}_{{d^\dagger F_{11R}^\dagger S_{12}^\dagger }}^{{f_2p_1p_2*}} \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_2*}}}{{M_{F_{11}}} {M_{S_{12}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{eQddH}} =
 \frac{16 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_5p_1p_2*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_2*}}}{{M_{V_{5}}^2}}
+\frac{16 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{p_1f_5p_2*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_2*}}}{{M_{V_{5}}^2}}
+\frac{16 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_5f_4p_2*}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{p_1f_1p_2*}}}{{M_{V_{5}}^2}}
-\frac{4 \mathcal{E}_{{dH^\dagger QV_{5}}}^{{f_4f_2p_1}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_5f_1p_1*}}}{{M_{V_{5}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{E}_{{d^\dagger eHV_{8}}}^{{f_5f_1p_1*}}}{{M_{V_{8}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_5f_1p_1*}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_1p_2*}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_5p_1*}} \mathcal{D}_{{eF_{10R}^\dagger V_{8}}}^{{f_1p_1p_2*}}}{{M_{F_{10}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{D}_{{d^\dagger F_{3L}^\dagger V_{8}}}^{{f_5p_1p_2*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_1}}}{{M_{F_{3}}} {M_{V_{8}}^2}}
+\frac{4 i \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_2}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_5p_1p_2*}} {y}_{{e}}^{{f_1p_1*}}}{{M_{V_{8}}^2}}
+\frac{8 \mathcal{E}_{{d^\dagger d^\dagger HS_{13}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{13}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger F_{3R}^\dagger H^\dagger }}^{{f_1p_2}} \mathcal{D}_{{F_{3L}QS_{11}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{3}}} {M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger F_{8L}S_{11}^\dagger }}^{{f_1p_2p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{S_{11}}^2}}
-\frac{8 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{E}_{{e^\dagger H^\dagger QS_{11}^\dagger }}^{{f_1f_2p_1}}}{{M_{S_{11}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger d^\dagger S_{11}^\dagger }}^{{f_5f_4p_1*}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_2}} \mathcal{C}_{{HS_{11}S_{13}^\dagger }}^{{p_1p_2*}}}{{M_{S_{11}}^2} {M_{S_{13}}^2}}
+\frac{16 i \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_5f_4p_2*}} {y}_{{e}}^{{f_1p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{p_1f_2p_2}}}{{M_{V_{5}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_5p_2*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_2f_2p_1*}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger eV_{5}}}^{{f_4f_1p_1*}} \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_5p_2p_1*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
-\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{d^\dagger F_{10R}^\dagger S_{13}^\dagger }}^{{f_5p_1p_2*}} \mathcal{D}_{{e^\dagger QS_{13}^\dagger }}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{13}}^2}} 
\end{autobreak}
\end{align}
\begin{align}
\begin{autobreak}
 {O_{LdQQH}} =
 
-\frac{4 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger LV_{8}D}}^{{f_4f_5p_2*}} \mathcal{D}_{{dQV_{8}}}^{{p_1f_1p_2}}}{{M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_2p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_1}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{13L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{13}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{13L}QS_{12}}}^{{p_2f_1p_1}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{13}}} {M_{S_{12}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_1p_1}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{1}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{1}^\dagger QV_{8}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{1}}} {M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_1p_1}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{2 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{5}HL}}^{{p_2f_5*}} \mathcal{D}_{{F_{5}^\dagger QV_{8}^\dagger }}^{{p_2f_2p_1}}}{{M_{F_{5}}} {M_{V_{8}}^2}}
-\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{D}_{{F_{8L}L^\dagger V_{8}^\dagger }}^{{p_2f_5p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{V_{8}}^2}}
+\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{D}_{{F_{8L}QS_{12}}}^{{p_2f_1p_1}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_2f_2}}}{{M_{F_{8}}} {M_{S_{12}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (1)}}^{{f_5f_2p_1}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (2)}}^{{f_5f_1p_1}}}{{M_{V_{8}}^2}}
-\frac{4 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{E}_{{H^\dagger L^\dagger QV_{8}^\dagger (2)}}^{{f_5f_2p_1}}}{{M_{V_{8}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{E}_{{H^\dagger QQS_{12}(1)}}^{{f_1f_2p_1}}}{{M_{S_{12}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{E}_{{H^\dagger QQS_{12}(2)}}^{{f_2f_1p_1}}}{{M_{S_{12}}^2}}
-\frac{4 \mathcal{E}_{{dH^\dagger QV_{5}}}^{{f_4f_2p_1}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_1}}}{{M_{V_{5}}^2}}
-\frac{16 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{f_4p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{5}}^2}}
-\frac{16 i {y}_{{d}}^{{p_1f_2*}} \mathcal{E}_{{d^\dagger d^\dagger V_{5}^\dagger D}}^{{p_1f_4p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{5}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{5}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{10}}} {M_{V_{5}}^2}}
-\frac{32 \mathcal{D}_{{d^\dagger F_{8L}^\dagger V_{5}^\dagger }}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{8R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{8}}} {M_{V_{5}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{C}_{{HV_{5}^\dagger V_{8}}}^{{p_2p_1*}} \mathcal{D}_{{L^\dagger QV_{5}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{5}}^2} {M_{V_{8}}^2}}
-\frac{2 \mathcal{E}_{{dH^\dagger QV_{9}}}^{{f_4f_2p_1}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_1}}}{{M_{V_{9}}^2}}
+\frac{16 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_2p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{4 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_4p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_2}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dQV_{8}}}^{{f_4f_2p_1}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_1p_2}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
-\frac{4 \mathcal{E}_{{dH^\dagger QV_{9}}}^{{f_4f_1p_1}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_1}}}{{M_{V_{9}}^2}}
+\frac{32 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger Q^\dagger V_{9}^\dagger }}^{{p_1f_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{F_{10}}} {M_{V_{9}}^2}}
+\frac{8 \mathcal{D}_{{dF_{13L}V_{9}}}^{{f_4p_1p_2}} \mathcal{D}_{{F_{13R}^\dagger H^\dagger Q}}^{{p_1f_1}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{F_{13}}} {M_{V_{9}}^2}}
+\frac{16 \mathcal{D}_{{dQV_{8}}}^{{f_4f_1p_1}} \mathcal{C}_{{HV_{8}V_{9}^\dagger }}^{{p_1p_2*}} \mathcal{D}_{{L^\dagger QV_{9}^\dagger }}^{{f_5f_2p_2}}}{{M_{V_{8}}^2} {M_{V_{9}}^2}}
+\frac{2 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_4f_5p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_1}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_1f_2p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
+\frac{2 \mathcal{E}_{{d^\dagger HLS_{10}}}^{{f_4f_5p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_1}}}{{M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{10}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{F_{10}}} {M_{S_{10}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{1}S_{10}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{1}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{F_{1}}} {M_{S_{10}}^2}}
-\frac{4 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{10}S_{12}^\dagger }}^{{p_2p_1*}} \mathcal{D}_{{QQS_{10}}}^{{f_2f_1p_2}}}{{M_{S_{10}}^2} {M_{S_{12}}^2}}
-\frac{\mathcal{E}_{{d^\dagger HLS_{14}}}^{{f_4f_5p_1*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_1}}}{{M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
-\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
+\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_1f_2p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}}
+\frac{\mathcal{E}_{{d^\dagger HLS_{14}}}^{{f_4f_5p_1*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_1}}}{{M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger F_{10L}H}}^{{f_4p_1*}} \mathcal{D}_{{F_{10R}^\dagger LS_{14}}}^{{p_1f_5p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{F_{10}}} {M_{S_{14}}^2}}
+\frac{\mathcal{D}_{{d^\dagger F_{5}S_{14}}}^{{f_4p_1p_2*}} \mathcal{D}_{{F_{5}HL}}^{{p_1f_5*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{F_{5}}} {M_{S_{14}}^2}}
-\frac{2 \mathcal{D}_{{d^\dagger LS_{12}}}^{{f_4f_5p_1*}} \mathcal{C}_{{HS_{12}^\dagger S_{14}}}^{{p_1p_2*}} \mathcal{D}_{{QQS_{14}}}^{{f_2f_1p_2}}}{{M_{S_{12}}^2} {M_{S_{14}}^2}} 
\end{autobreak}
\end{align}


==> table/uv_op_correspondence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        ~ & $S_1$ & $S_2$ & $S_3$ & $S_4$ & $S_5$ & $S_6$ & $S_7$ & $S_8$ & $S_9$ & $S_{10}$ & $S_{11}$ & $S_{12}$ & $S_{13}$ & $S_{14}$ & $S_{15}$ & $S_{16}$ & $S_{17}$ & $S_{18}$ & $S_{19}$ \\ \hline
        ${\cal O}_{H}$ & \cmark & ~ & ~ & \cmark & \cmark & \cmark & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{H\square}$ & \cmark & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{HD}$ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{eH}$ & \footnote{S4/F2/3} & ~ & ~ & \cmark & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{uH}$ & \footnote{S4/F9/11} & ~ & ~ & \cmark & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{dH}$ & \footnote{S4/F8/11} & ~ & ~ & \cmark & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hl}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hl}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{He}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hq}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hq}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hd}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{Hud}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ll}$ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qq}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & \cmark & ~ & \cmark & ~ \\ \hline
        ${\cal O}_{qq}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & \cmark & ~ & \cmark & ~ \\ \hline
        ${\cal O}_{lq}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{lq}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ee}$ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{uu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{dd}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{eu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ed}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ud}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ud}^{(8)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ \\ \hline
        ${\cal O}_{le}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{lu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ld}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qe}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qu}^{(1)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark \\ \hline
        ${\cal O}_{qu}^{(8)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark \\ \hline
        ${\cal O}_{qd}^{(1)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark \\ \hline
        ${\cal O}_{qd}^{(8)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark \\ \hline
        ${\cal O}_{ledq}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{quqd}^{(1)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ \\ \hline
        ${\cal O}_{quqd}^{(8)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & \cmark \\ \hline
        ${\cal O}_{lequ}^{(1)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{lequ}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{duq}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qqu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qqq}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{duu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
    \end{tabular}
    }
    \caption{The correspondence between dimension-6 operators in SMEFT and single-scalar-extended UV models. Check mark inside each box means that the operator to the left can be generated by introducing the new resonance above. Note that the operators with star mark in the $S_1$ column cannot generated by an $S_1$ extended model. ${\cal O}_{eH}$, ${\cal O}_{uH}$ and ${\cal O}_{uH}$ need $S_1$ with $S_4/F_2/F_3$, $S_4/F_9/F_{11}$ and $S_4/F_8/F_{11}$ respectively.}
    \label{tab:uvop/scalar}
\end{table}

\begin{table}
    \centering
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        ~ & $F_1$ & $F_2$ & $F_3$ & $F_4$ & $F_5$ & $F_6$ & $F_7$ & $F_8$ & $F_9$ & $F_{10}$ & $F_{11}$ & $F_{12}$ & $F_{13}$ & $F_{14}$ \\ \hline
        % ${\cal O}_{H}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{H\square}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{HD}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{eH}$ & ~ & \cmark & \cmark & \cmark & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{uH}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark & \cmark & \cmark & \cmark \\ \hline
        ${\cal O}_{dH}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark & \cmark & ~ & \cmark & \cmark \\ \hline
        ${\cal O}_{Hl}^{(1)}$ & \cmark & \cmark & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hl}^{(3)}$ & \cmark & \cmark & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{He}$ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hq}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & \cmark & \cmark \\ \hline
        ${\cal O}_{Hq}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & \cmark & \cmark \\ \hline
        ${\cal O}_{Hu}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{Hd}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hud}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ \\ \hline
    \end{tabular}
    }
    \caption{The correspondence between dimension-6 operators in SMEFT and single-fermion-extended UV models. The notation is the same as Tab.\,\ref{tab:uvop/scalar}.}
    \label{tab:uvop/fermion}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
        ~ & $V_1$ & $V_2$ & $V_3$ & $V_4$ & $V_5$ & $V_6$ & $V_7$ & $V_8$ & $V_9$ & $V_{10}$ & $V_{11}$ & $V_{12}$ & $V_{13}$ & $V_{14}$ \\ \hline
        ${\cal O}_{H}$ & ~ & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{H\square}$ & \cmark & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{HD}$ & \cmark & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{eH}$ & \cmark & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{uH}$ & \cmark & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{dH}$ & \cmark & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hl}^{(1)}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hl}^{(3)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{He}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hq}^{(1)}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hq}^{(3)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hu}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hd}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{Hud}$ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ll}$ & \cmark & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qq}^{(1)}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark \\ \hline
        ${\cal O}_{qq}^{(3)}$ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark \\ \hline
        ${\cal O}_{lq}^{(1)}$ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{lq}^{(3)}$ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ee}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{uu}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{dd}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{eu}$ & \cmark & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ed}$ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ud}^{(1)}$ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ \\ \hline
        ${\cal O}_{ud}^{(8)}$ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ \\ \hline
        ${\cal O}_{le}$ & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{lu}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{ld}$ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qe}$ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qu}^{(1)}$ & \cmark & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qu}^{(8)}$ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{qd}^{(1)}$ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qd}^{(8)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark & ~ & \cmark & ~ & ~ \\ \hline
        ${\cal O}_{ledq}$ & ~ & ~ & ~ & ~ & \cmark & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{quqd}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{quqd}^{(8)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{lequ}^{(1)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        % ${\cal O}_{lequ}^{(3)}$ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{duq}$ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & \cmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        ${\cal O}_{qqu}$ & ~ & ~ & ~ & ~ & ~ & ~ & \cmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
    \end{tabular}
    }
    \caption{The correspondence between dimension-6 operators in SMEFT and single-vector-extended UV models. The notation is the same as Tab.\,\ref{tab:uvop/scalar}.}
    \label{tab:uvop/vector}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}
%     \centering
%     %  \resizebox{\textwidth}{0.5\textheight}{
%     \begin{tabular}{|c|c|c|c|c|}
%         \hline
%         % Operators
%         & $F_1$ & $S_6$ & $F_5$ & $S_8\&F_6$ \\
%         \hline
%         % $(H^\dagger H)^2$ & \xmark & \cmark & \xmark & \xmark\\
%         ${\cal O}_5$ & \cmark & \cmark & \cmark & \xmark\\
%         \hline
%         $\mathcal{O}_{H}$ & \xmark & \cmark & \xmark & \cmark \\
%         $\mathcal{O}_{H\Box}$ & \xmark & \cmark & \xmark & \xmark \\
%         $\mathcal{O}_{HD}$ & \xmark & \cmark & \xmark & \xmark \\
%         $\mathcal{O}_{eH}$ & \xmark & \cmark & \cmark & \xmark \\
%         $\mathcal{O}_{uH}$ & \xmark & \cmark & \xmark & \xmark \\
%         $\mathcal{O}_{dH}$ & \xmark & \cmark & \xmark & \xmark \\
%         ${\cal O}_{Hl}^{(1)}$ & \cmark & \xmark & \cmark & \cmark  \\
%         ${\cal O}_{Hl}^{(3)}$ & \cmark & \xmark & \cmark & \cmark  \\
%         $\mathcal{O}_{ll}$ & \xmark & \cmark & \xmark & \xmark \\
%         \hline
%         % \multicolumn{5}{|c|}{{\bf $d = 7$}} \\
%         % \hline
%         ${\cal O}_{LH}$ & \cmark & \cmark & \cmark & \cmark \\
%         ${\cal O}_{LeHD}$ & \cmark & \xmark & \cmark & \xmark \\
%         ${\cal O}_{LHD1}$ & \xmark & \cmark & \cmark & \xmark \\
%         ${\cal O}_{LHD2}$ & \cmark & \cmark & \cmark & \xmark \\
%         ${\cal O}_{LHW}$ & \cmark & \xmark & \cmark & \xmark \\
%         % ${\cal O}_{LHB}$ & \xmark & \xmark & \xmark & \xmark \\
%         ${\cal O}_{eLLLH}$ & \cmark & \xmark & \cmark & \xmark \\
%         ${\cal O}_{dLQLH1}$ & \cmark & \xmark & \cmark & \xmark \\
%         ${\cal O}_{dLQLH2}$ & \cmark & \xmark & \cmark & \xmark \\
%         ${\cal O}_{QuLLH}$ & \cmark & \xmark & \cmark & \xmark \\
%         \hline
%     \end{tabular}
%     \caption{table}\label{tab:uvop/vmass}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{ll}
%         \hline
%         $S_2$ & ${\cal O}_{eLLLH} (S_4),~ {\cal O}_{dLQLH2} (S_4),~ {\cal O}_{QuLLH} (S_4)$ \\
%         $S_4$ & ${\cal O}_{eLLLH} (S_2/S_6),~ {\cal O}_{dLQLH1} (S_6),~ {\cal O}_{dLQLH2} (S_2/S_6),~ {\cal O}_{QuLLH} (S_2/S_6)$ \\
%         $S_6$ & ${\cal O}_{eLLLH} (S_6),~ {\cal O}_{dLQLH1} (S_6),~ {\cal O}_{dLQLH2} (S_6),~ {\cal O}_{QuLLH} (S_6)$ \\
%         $F_1$ & ${\cal O}_{LeHD} (F_3)$ \\
%         $F_3$ & ${\cal O}_{LeHD} (F_1/F_5)$ \\
%         $F_5$ & ${\cal O}_{LeHD} (F_3)$ \\
%         $V_2$ & ${\cal O}_{LeHD} (V_3),~ {\cal O}_{dLueH} (V_3)$ \\
%         $V_3$ & ${\cal O}_{LeHD} (V_2),~ {\cal O}_{dLueH} (V_2)$ \\
%         $V_5$ & ${\cal O}_{dLueH} ({\color{red} V_8}),~ {\cal O}_{QuLLH} ({\color{red} V_8})$ \\
%         ${\color{red} V_8}$ & ${\cal O}_{dLueH} (V_5),~ {\cal O}_{QuLLH} (V_5/V_9)$ \\
%         $V_9$ & ${\cal O}_{QuLLH} ({\color{red} V_8})$ \\
%         \hline
%     \end{tabular}
%     \caption{Scalars}
%     \label{tab:uvop/lnvpure}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{ll}
%         \hline
%          $F_1$ & ${\cal O}_{LeHD} (V_2),~ {\cal O}_{eLLLH} (S_2),~ {\cal O}_{dLQLH1} (S_4/S_{12}),~ {\cal O}_{dLQLH2} (S_4),~ {\cal O}_{dLueH} (V_2/V_5),~ {\cal O}_{QuLLH} (S_4/V_5)$ \\
%          $F_3$ & ${\cal O}_{LeHD} (S_6/V_2),~ {\cal O}_{dLueH} (S_{12}/V_2)$ \\
%          $F_4$ & ${\cal O}_{eLLLH} (S_2/S_6)$ \\
%          $F_5$ & ${\cal O}_{LeHD} (S_6),~ {\cal O}_{eLLLH} (S_4/S_6),~ {\cal O}_{dLQLH1} (S_4/S_{12}),~ {\cal O}_{dLQLH2} (S_4/S_{12}),~ {\cal O}_{QuLLH} (S_4/V_9)$ \\
%          $F_8$ & \\
%          $F_9$ &  \\
%          $F_10$ & \\
%          $F_12$ &  \\
%          $F_13$ &  \\
%          $F_14$ &   \\
%         \hline
%     \end{tabular}
%     \caption{Scalars}
%     \label{tab:uvop/lnvmix}
% \end{table}

%%% LNV op w/ vmass op

\begin{table}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & ${\cal O}_5$ & ${\cal O}_{LH}$ & ${\cal O}_{LeHD}$ & ${\cal O}_{LHD1}$ & ${\cal O}_{LHD2}$ & ${\cal O}_{LHW}$ & ${\cal O}_{eLLLH}$ & ${\cal O}_{dLQLH1}$ & ${\cal O}_{dLQLH2}$ & ${\cal O}_{dLueH}$ & ${\cal O}_{QuLLH}$ \\
        \hline 
        $S_2$ & & & & & & & $S_4/F_4$ & & $S_4/F_9/F_{10}$ & & $S_4/F_8/F_{12}$ \\
        \hline 
        $S_4$ & & & & & & & $S_2/S_6$ & $S_6$ & $S_2/S_6$ & & $S_2/S_6$ \\
        \hline
        $S_6$ & \cmark & \cmark & $F_3$ & \cmark & \cmark & & $S_4/F_4$ & $S_4/F_{10}/F_{14}$ & $S_4/F_{10}/F_{14}$ & & $S_4/F_{12}/F_{13}$ \\
        \hline
        $S_8$ & & $F_6$ & & & & & & & & & \\
        \hline
        $S_{12}$ & & & & & & & & $F_{14}$ & $F_9/F_{14}$ & $F_3/F_{12}$ & \\
        \hline
        $F_1$ & \cmark & \cmark & \cmark & & \cmark & \cmark & \cmark & \cmark & \cmark & $V_2/V_5$ & \cmark \\
        \hline
        $F_3$ & & & $S_6/V_2$ & & & & & & & $S_{12}/V_2$ & \\
        \hline
        $F_4$ & & & & & & & $S_2/S_6$ & & & &\\
        \hline
        $F_5$ & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & & \cmark \\
        \hline
        $F_6$ & & $S_8$ & & & & & & & & & \\
        \hline
        $F_8$ & & & & & & & & & & & $S_2$ \\
        \hline
        $F_9$ & & & & & & & & & $S_2/S_{12}$ & & \\
        \hline
        $F_{10}$ & & & & & & & & $S_6$ & $S_2/S_{6}$ & $V_3$ & \\
        \hline
        $F_{12}$ & & & & & & & & & & $S_{12}/V_3/V_5$ & $S_2/S_6/V_5/V_9$ \\
        \hline
        $F_{13}$ & & & & & & & & & & & $S_6$ \\
        \hline
        $F_{14}$ & & & & & & & & $S_6/S_{12}$ & $S_6/S_{12}$ & & \\
        \hline
        $V_2$ & & & $F_3/V_3$ & & & & & & & $F_1/F_3/V_3$ & \\
        \hline
        $V_3$ & & & $V_2$ & & & & & & & $F_{10}/F_{12}/V_2$ & \\
        \hline
        $V_5$ & & & & & & & & & & $F_1/F_{12}$ & $F_{12}$ \\
        \hline
        $V_9$ & & & & & & & & & & & $F_{12}$ \\
        \hline
    \end{tabular}
    }
    \caption{The correspondence between dimension-5 and -7 LNV operators in SMEFT and UV resonances. Only models conserving baryon number are listed here. Every box with check mark denotes that the operator above can be generated by introducing a single resonance to the left, while boxes with resonances means that the operator above needs both the resonance to the left and one of the resonance inside the box.}
    \label{tab:uvop/lnv}
\end{table}

%%% LNV op w/o vmass op

% \begin{table}
%     \centering
%     \resizebox{0.95\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%         \hline
%         & ${\cal O}_{LeHD}$ & ${\cal O}_{eLLLH}$ & ${\cal O}_{dLQLH1}$ & ${\cal O}_{dLQLH2}$ & ${\cal O}_{dLueH}$ & ${\cal O}_{QuLLH}$ \\
%         \hline 
%         $S_2$ & & $S_4/F_1/F_4$ & & $S_4/F_9/F_{10}$ & & $S_4/F_8/F_{12}$ \\
%         \hline 
%         $S_4$ & & $S_2/S_6/F_5$ & $S_6/F_1/F_5$ & $S_2/S_6/F_1/F_{5}$ & & $S_2/S_6/F_1/F_{5}$ \\
%         \hline
%         $S_6$ & $F_3/F_5$ & $S_4/F_4/F_5$ & $S_4/F_{10}/F_{14}$ & $S_4/F_{10}/F_{14}$ & & $S_4/F_{12}/F_{13}$ \\
%         \hline
%         $S_{12}$ & & & $F_1/F_5/F_{14}$ & $F_5/F_9/F_{14}$ & $F_3/F_{12}$ & \\
%         \hline
%         $F_1$ & $F_3/V_2$ & $S_2$ & $S_4/S_{12}$ & $S_4$ & $V_2/V_5$ & $S_4/V_5$ \\
%         \hline
%         $F_3$ & $S_6/F_1/F_5/V_2$ & & & & $S_{12}/V_2$ & \\
%         \hline
%         $F_4$ & & $S_2/S_6$ & & & &\\
%         \hline
%         $F_5$ & $S_6/F_3$ & $S_4/S_6$ & $S_4/S_{12}$ & $S_4/S_{12}$ & & $S_4/V_9$ \\
%         \hline
%         $F_8$ & & & & & & $S_2$ \\
%         \hline
%         $F_9$ & & & & $S_2/S_{12}$ & & \\
%         \hline
%         $F_{10}$ & & & $S_6$ & $S_2/S_{6}$ & $V_3$ & \\
%         \hline
%         $F_{12}$ & & & & & $S_{12}/V_3/V_5$ & $S_2/S_6/V_5/V_9$ \\
%         \hline
%         $F_{13}$ & & & & & & $S_6$ \\
%         \hline
%         $F_{14}$ & & & $S_6/S_{12}$ & $S_6/S_{12}$ & & \\
%         \hline
%         $V_2$ & $F_1/F_3/V_3$ & & & & $F_1/F_3/V_3$ & \\
%         \hline
%         $V_3$ & $V_2$ & & & & $F_{10}/F_{12}/V_2$ & \\
%         \hline
%         $V_5$ & & & & & $F_1/F_{12}$ & $F_1/F_{12}$ \\
%         \hline
%         % ${\color{red} V_8}$ & & & & & $V_5$ & $V_5/V_9$ \\
%         % \hline
%         $V_9$ & & & & & & $F_5/F_{12}$ \\
%         \hline
%     \end{tabular}
%     }
%     \caption{UV Completion of LNV operators.}
%     \label{tab:uvop/lnv}
% \end{table}

%%% BNVo p & LNV op

\begin{table}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        & ${\cal O}_{dLQLH1}$ & ${\cal O}_{dLQLH2}$ & ${\cal O}_{dLueH}$ & ${\cal O}_{QuLLH}$ & ${\cal O}_{LdudH}$ & ${\cal O}_{LdddH}$ & ${\cal O}_{eQddH}$ & ${\cal O}_{LdQQH}$ \\
        \hline 
        ${\color{red} S_{10}}$ & $S_{12}/F_1/F_{10}$ & $S_{12}/F_1/F_{10}$ & $S_{12}/F_1/F_{10}$ & & $S_{12}/F_1/F_{10}$ & & & $S_{12}/F_1/F_{10}$ \\
        \hline 
        $S_{11}$ & & & & & $S_{13}/F_{1}/F_{11}$ & $S_{12}/F_2/F_{11}$ & $S_{13}/F_3/F_8$ & \\
        \hline
        $S_{12}$ & ${\color{red} S_{10}}/{\color{red} S_{14}}$ & ${\color{red} S_{10}}/{\color{red} S_{14}}$ & ${\color{red} S_{10}}$ & & ${\color{red} S_{10}}/F_{10}/F_{11}$ & $S_{11}/F_{11}$ & & ${\color{red} S_{10}}/{\color{red} S_{14}}/F_8/F_{13}$ \\
        \hline
        $S_{13}$ & & & & & $S_{11}/F_{10}$ & & $S_{11}/F_{10}$ & \\
        \hline
        ${\color{red} S_{14}}$ & $S_{12}/F_5/F_{10}$ & $S_{12}/F_5/F_{10}$ & & & & & & $S_{12}/F_5/F_{10}$ \\
        \hline
        $F_1$ & ${\color{red} S_{10}}$ & ${\color{red} S_{10}}$ & ${\color{red} S_{10}}$ & ${\color{red} V_8}$ & ${\color{red} S_{10}}/S_{11}$ & & & ${\color{red} S_{10}}/{\color{red} V_8}$ \\
        \hline
        $F_2$ & & & & & & $S_{11}$ & & \\
        \hline
        $F_3$ & & & ${\color{red} V_8}$ & & & & $S_{11}/{\color{red} V_8}$ & \\
        \hline
        $F_5$ & ${\color{red} S_{14}}$ & ${\color{red} S_{14}}$ & & ${\color{red} V_8}$ & & & & ${\color{red} S_{14}}/{\color{red} V_8}$ \\
        \hline
        $F_8$ & & & & ${\color{red} V_8}$ & & & $S_{11}/V_5$ & $S_{12}/V_5/{\color{red} V_8}$ \\
        \hline
        $F_{10}$ & ${\color{red} S_{10}}/{\color{red} S_{14}}$ & ${\color{red} S_{10}}/{\color{red} S_{14}}$ & ${\color{red} S_{10}}/{\color{red} V_8}$ & & ${\color{red} S_{10}}/S_{12}/S_{13}$ & & $S_{13}/V_5/{\color{red} V_8}$ & ${\color{red} S_{10}}/{\color{red} S_{14}}/V_{5}/V_{9}$ \\
        \hline
        $F_{11}$ & & & & & $S_{11}/S_{12}$ & $S_{11}/S_{12}$ & & \\
        \hline
        $F_{13}$ & & & & ${\color{red} V_8}$ & & & & $S_{12}/{\color{red} V_8}/V_9$ \\
        \hline
        $V_5$ & & & ${\color{red} V_8}$ & ${\color{red} V_8}$ & & & $F_8/F_{10}/{\color{red} V_8}$ & $F_8/F_{10}/{\color{red} V_8}$ \\
        \hline
        ${\color{red} V_8}$ & & & $F_3/F_{10}/V_5$ & \makecell{$F_1/F_5/F_8/$\\$F_{13}/V_5/V_9$} & & & $F_3/F_{10}/V_5$ & \makecell{$F_1/F_5/F_8/$\\$F_{13}/V_5/V_9$} \\
        \hline
        $V_9$ & & & & ${\color{red} V_8}$ & & & & $F_{10}/F_{13}/{\color{red} V_8}$ \\
        \hline
    \end{tabular}
    }
    \caption{The correspondence between dimension-7 operators in SMEFT and UV resonances. Models listed here all violate baryon number. Models with resonances marked with red can generate dimension-6 baryon number violating operators. Other notation is the same as Tab.\,\ref{tab:uvop/lnv}.}
    \label{tab:uvop/bnv}
\end{table}
